Semi-supervised learning for medical image classification using imbalanced training data

Medical image classification is often challenging for two reasons: a lack of labelled examples due to expensive and time-consuming annotation protocols, and imbalanced class labels due to the relative scarcity of disease-positive individuals in the wider population. Semi-supervised learning (SSL) methods exist for dealing with a lack of labels, but they generally do not address the problem of class imbalance. In this study we propose Adaptive Blended Consistency Loss (ABCL), a drop-in replacement for consistency loss in perturbation-based SSL methods. ABCL counteracts data skew by adaptively mixing the target class distribution of the consistency loss in accordance with class frequency. Our experiments with ABCL reveal improvements to unweighted average recall on two different imbalanced medical image classification datasets when compared with existing consistency losses that are not designed to counteract class imbalance.

==> Paper arxiv/Section/abstract.tex <==
Medical image classification is often challenging for two reasons: a lack of labelled examples due to expensive and time-consuming annotation protocols, and imbalanced class labels due to the relative scarcity of disease-positive individuals in the wider population. Semi-supervised learning (SSL) methods exist for dealing with a lack of labels, but they generally do not address the problem of class imbalance. In this study we propose Adaptive Blended Consistency Loss (ABCL), a drop-in replacement for consistency loss in perturbation-based SSL methods. ABCL counteracts data skew by adaptively mixing the target class distribution of the consistency loss in accordance with class frequency. Our experiments with ABCL reveal improvements to unweighted average recall on two different imbalanced medical image classification datasets when compared with existing consistency losses that are not designed to counteract class imbalance.




==> Paper arxiv/Section/acknowledgements.tex <==
\section*{Acknowledgements}
\para This research did not receive any specific grant from funding agencies in the public, commercial, or not-for-profit sectors.


==> Paper arxiv/Section/background.tex <==

~\section{Supervised versus Unsupervised Learning}
\para In the era of the digital world, machine learning has been playing a crucial role across many different industries and research fields such as medical research, biology, robotics, manufacturing, etc. Machine learning has been used to solve numerous problems and achieved  near human accuracy. Moreover, beyond the limitation of computation and amount of data, machine learning becomes a more powerful technique than ever. Machine learning is a subset of artificial intelligence which trains  models using data rather than explicit instructions in order to map inputs to outputs or make decisions~\cite{matthias2001learning}. Machine learning is mainly divided into three branches: supervised learning, unsupervised learning and reinforcement learning. To confine the scope of this literature survey, we will only discuss supervised and unsupervised learning. In supervised learning, a learnt model takes input data and predicts the output. The model learns the mapping from the input to the output by comparing the predicted output against the desired output. Importantly, the key requirement of supervised learning is that for every training sample, an input and desired output (known as the label) pair is provided. So, to make supervised models perform well, it is necessary to gather a large amount of labelled data. Moreover, two main categories of supervised learning are classification and regression. For classification, the output of the model should be a categorical class label. For regression, the goal is to output a numerical value. 

Another important branch of machine learning is unsupervised learning, which instead of knowing the explicit output label, it only receives the input data. The two important techniques of unsupervised learning are clustering and dimensionality reduction. The common goal of clustering is to find the pattern of a set of data points and cluster them into a group. Dimensionality reduction is the process of reducing the number of features or variables, also known as the dimension, in a dataset without impacting on the meaning of the data.
~\section{Semi-Supervised Learning}
\para The brief review of the two popular paradigms of both supervised and unsupervised learning exposes different shortcomings, for supervised learning it is expensive to obtain a large amounts of labelled data and for unsupervised learning it is hard to extract the meaningful information from unlabelled data. Thus, one promising paradigm that overcomes these obstacles is semi-supervised learning (SSL)~\cite{chapelle2009semi} which makes use of a small amount of labelled and a large amount of unlabelled data to optimize the training of models. The goal of semi-supervised learning is to learn patterns from unlabelled data and augment the prediction of the model by these patterns. More intuitively, by leveraging the unlabelled data, the model produces a better decision boundary for different classes which reflects the data’s underlying structure ~\cite{oliver2018realistic}. Over the history of machine learning, researchers have invented various approaches to semi-supervised learning which mostly refer to either transductive learning or inductive learning. Specifically, given the data set of labelled ($x_{L}$,$y_{L}$) and unlabelled $x_{U}$ data, the objective of the inductive learner is to make the prediction for any data points, whereas the transductive learner will only produce the label for unlabelled data points. In the broad perspective, the inductive semi-supervised learning generalise a model that can output the label for unseen instances, on the other hand, transductive semi-supervised learning is only able to make the label for unlabelled data, known instances, during training phase~\cite{van2020survey}. Figure~\ref{fig:SSLTaxonomy} 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLTaxonomy}
	\caption{Visualization of the semi-supervised taxonomy~\cite{van2020survey}.}
	\label{fig:SSLTaxonomy}
\end{figure}

~\section{Convolutional Neural Network For Image Classification}
\label{sec:cnn}
\para Computer vision is one of the most important domains for the application of machine learning and includes various tasks such as object detection~\cite{zhao2019object} or image classification~\cite{krizhevsky2012imagenet}, etc. Recently, many researchers have achieved state of the art results for these tasks on public datasets such as ImageNet~\cite{deng2009imagenet}, CIFAR 10 or  CIFAR 100~\cite{krizhevsky2009learning}. To achieve such successful results, almost all of them have used one breakthrough type of neural networks, called Convolutional Neural Networks (CNNs)~\cite{lecun1990handwritten,lecun1998gradient}. This type of model has the ability to help the machine understand the representation of image better and also automatically learn features from the image.
\begin{figure}
	\centering
	\includegraphics[width=.8\textwidth]{CNN}
	\caption{Inside Convolutional Neural Networks ~\cite{lecun2015deep}.}
	\label{fig:CNN}
\end{figure}

Specifically, the architecture of CNNs is designed as a series of blocks and followed by a classification module~\cite{lecun2010convolutional}. Each block contains three layers: filter bank layer, non-linearity layer and pooling layer. In addition, the main characteristic of CNNs is the feature map which is the input and output of layers in each block. For example in Figure~\ref{fig:CNN}, the very first layer receives the RGB image of a dog and outputs features of the image such as eyes, ears, etc. The filter bank layer is a set of filters, which are matrices of weights having dimensions (width,height) or (width,height,depth) corresponding to input of black and white image or color image respectively. Each filter scans through the image and makes the sum of element-wise operation with each scanned portion of the image. Intuitively, the filter is a window, which slides horizontally from top left to bottom right of the image and returns the feature map output, as shown in Figure~\ref{fig:FilterOperation}. In addition, the filter often is called a feature detector and its weights sometimes is predefined to reflect what features it wants to detect such as vertical or horizontal edge.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{FilterOperation}
	\caption{The example of filter over the image~\cite{yamashita2018convolutional}.}
	\label{fig:FilterOperation}
\end{figure}

Moreover, two important settings of filter banks are padding and stride. Padding is the process of adding zero pixels around the border of an image. Sometimes, the filter does not fit well with the image, that means the filter would be missing some parts of the image. Thus, doing padding into the image makes sure the filter captures all the information from the image. Stride is the number of pixels indicating how far the filter should move from current position on the image. The output of the filter bank layer is the input of the non-linearity layer which consists of an activation function. Most researchers use the Rectified Non-Linear Unit (ReLU)~\cite{nair2010rectified} which returns the direct input if it is not negative, otherwise returns zero. The purpose of non-linear activation function is to prevent the model from becoming a linear model and help the model to deal with the complex task. The last layer of CNNs block is the pooling layer which also uses the approach of scanning images. It applies the specific function with the filter size (width,height) as the parameter such as max pooling, average pooling or sum pooling onto every region of feature maps. For example, applying max pooling with the filter size 2x2, the function will output the highest value of a specific region. That means, pooling layer can reduce the dimensionality of feature maps and also keep the most important information out of the region. In the higher level view, the two key benefits of CNNs are parameter sharing and sparsity of connections. With parameter sharing, a filter bank is useful in one part of the image and is probably useful in another part, thus it can reduce the parameter needed. With sparsity of connections, in each layer, each output value depends only on a small number of inputs.

Lastly, all feature maps captured from a series of blocks are flatten out into input units and fed into the classification module, called fully connected layer. This layer is like a normal neural network which outputs the score for each class. CNNs are normally back-propagated as neural networks and noticeably the weight of filters also be trained. 

~\section{Deep learning for semantic segmentation}
Image segmentation can be divided into two main tasks of semantic segmentation and instance segmentation. Semantic segmentation techniques label each pixel of an image with the class it belongs to. For example, label a pixel as belonging to a tumor or the background. Instance segmentation extends semantic segmentation by further separating  pixels based on if they belong to different instances of  the same class. Figure ~\ref{fig:Segmentation} shows an example of 2 types of segmentation.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{Segmentation}
	\caption{An example of semantic and instance segmentation~\cite{kirillov2019panoptic}.}
	\label{fig:Segmentation}
\end{figure}

From the earliest days, image segmentation techniques have centralized on traditional algorithms such as thresholding, region-growing, k-means clustering, etc. However, due to the success of deep learning models (especially CNNs), image segmentation methods have significantly improved in accuracy   via CNN based methods such as DeepLab ~\cite{chen2014semantic}, U-Net~\cite{ronneberger2015u}. To confine the scope of this review, we will focus our attention on semantic segmentation methods that use deep learning models.

As discussed in Section ~\ref{sec:cnn}, CNNs are a dominant approach in computer vision, especially in the image classification task with the ability to automatically learn features and output the class prediction for the entire image (global prediction). Therefore, researchers have adapted the deep CNN approach to solve the semantic segmentation task by making it output the class prediction for each pixel of the image (local prediction), known as the prediction mask.  Early methods  used CNNs to classify the  center pixel for a given patch of input~\cite{ciresan2012deep}. The image patch is slid across the image in order to output a prediction for each pixel of the image thus achieving the required output for semantic segmentation.  However this approach  is not efficient since the same CNN kernel is applied to the overlapping regions of nearby patches multiple times.

In order to improve the efficiency of applying CNNs to semantic segmentation, an intuitive idea ~\cite{long2015fully} is  to use fully convolutional neural networks  to process the entire image in a single pass through the CNN. To do so, the CNN architecture is modified to keep the output  size the same as the input image by using downsampling and upsampling layers within a fully convolutional neural network. This idea not only brings computational efficiency by downsampling layers but also produces the required output size using the  upsampling layers. Moreover, the approach can obtain the global spatial information of the image. Due to their  effectiveness and efficiency, fully convolutional neural networks are used in all current state of the art semantic segmentation methods. 

~\subsection{Popular existing models}
~\subsubsection{Fully convolutional networks}
Long et al ~\cite{long2015fully} proposed a fully convolutional model by modifying existing state of the art CNN classification models such as VCG16, GoogleNet. The author replaced fully connected layers with fully convolutional layers including up-sampling layers. It allows the model to process an arbitrary input image size and produce a prediction mask of the same size as the input. Figure ~\ref{fig:FCN} illustrates the model. Notably, up-sampling layers include learnable deconvolution filters that up-sampling is performed using bilinear interpolation.  Additionally, to refine semantics and spatial accuracy of the output, the author used skip of connections which combines the coarse,  high level information of feature maps in middle layers with the lower level information from the earlier layers, Figure ~\ref{fig:SkipConnection}. The methods achieved 67.2$\%$ mean IoU on PASCAL VOC 2012 ~\cite{everingham2011pascal} dataset  , establishing a new state of the art result at the time.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{FCN}
	\caption{Fully convolutional networks for semantic segmentation.~\cite{long2015fully} }
	\label{fig:FCN}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SkipConnection}
	\caption{ Skip connections : allows the model to use high level information from the middle layers to inform the final fine grained predictions.~\cite{long2015fully} }
	\label{fig:SkipConnection}
\end{figure}

~\subsubsection{ Deconvolution Network (DeConvNet)}
The Deconvolution Network (DeConvNet) is another well-known CNN based model for pixel-wise segmentation which is inspired by encoder-decoder networks. Noh et al. ~\cite{noh2015learning} have proposed a novel segmentation network consisting of the convolution network (acts like an encoder network that encodes an input image into a vector of features) and the deconvolution network (acts like an decoder network) that transforms the encoding vector of features to a dense pixel-wise class prediction map of the same size as the original image. The model architecture for DeConvNet is shown in Figure~\ref{fig:DeConvNet}. Notably, the convolution network (encoder) is not fully convolutional because it includes 2 fully connected layers which are augmented at the end to impose class-specific projection.The highlight part of this study is the deconvolution network which contains a sequence of trainable deconvolution, unpooling and rectified linear units (RELU) layers. The motivation for proposing a complete deconvolution network is the absence of real deconvotion in previous models (FCNs~\cite{long2015fully}) which is one of the main limitations. The network achieved 72.5$\%$ on PASCAL VOC 2012 dataset and outperformed all rival networks at the time.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeConvNet}
	\caption{ Overall architecture of the deconvolution network, based on the VGG 16-layer CNN model ~\cite{noh2015learning}}
	\label{fig:DeConvNet}
\end{figure}

~\subsubsection{SegNet}
Badrinarayanan et al.~\cite{badrinarayanan2017segnet} proposed an interesting fully deep convolutional Encoder-Decoder network for image segmentation, named SegNet. The network architecture is quite similar to DeconvNet which consist of the convolution network (encoder) and deconvolution network (decoder), however the author removes 2 fully connected layers of the VGG16 encoder network to make SegNet become fully convolutional. The novelty of SegNet is how the decoder network upsamples the feature maps from the encoder network. Specifically, the decoder network uses pooling indices obtained in the max-pooling step of the corresponding encoder to perform unpooling like DeconvNet, but without learnable deconvolution filters. Therefore, the upsampling stage requires no learning. After each upsampling, the upsampled maps which are sparse are convolved with trainable filters to produce dense feature maps. The network is illustrated in Figure ~\ref{fig:SegNet}.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SegNet}
	\caption{ The SegNet network architecture.~\cite{badrinarayanan2017segnet} }
	\label{fig:SegNet}
\end{figure}

~\subsubsection{UNet}
So far we have discussed popular existing models for general image segmentation. In contrast the  UNet~\cite{ronneberger2015u} was initially proposed to solve medical image segmentation and then be used in general tasks.  Ronneberger et al. ~\cite{ronneberger2015u} built a U-shaped fully convolutional network for semantic segmentation comprising a contracting path (down-sampling) to capture the context and a symmetric expanding path (up-sampling) to localize objects. The contracting path architecture is similar to a typical convolution network which obtains feature maps and reduces its resolution. While the expanding path is deconvolution network-like, that upsamples feature maps. At every upsampling layer, by using the skip connections, upsampled feature maps and the correspondingly cropped feature maps from the contracting path are concatenated. Then these concatenated feature maps are convolved by two consecutive 3 x 3 convolutional filters to halve the number of channels, hence yields U-shape network, illustrated in Figure ~\ref{fig:UNet}. 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{UNet}
	\caption{ UNet network architecture. The left is the contracting path and the right is the expanding path.~\cite{ronneberger2015u}
	}
	\label{fig:UNet}
\end{figure}

~\subsubsection{DeepLab}
\label{sec:deeplab}
Chen et al. proposed a series of DeepLab models including DeepLabv1~\cite{chen2014semantic}, DeepLabv2~\cite{chen2017deeplab}, DeepLabv3~\cite{chen2017rethinking} and DeepLabv3+~\cite{chen2018encoder}, which have become one of the most popular models for semantic segmentation.
DeepLabv1 uses a fully convolutional neural network architecture  (with VGG 16 as backbone) for semantic segmentation.  It has the two important features which are dilated convolutions in the convolutional layers and fully connected Conditional Random Field (CRF) (probabilistic graphical model) at the output stage. With no extra computational cost, dilated convolutions enlarge the receptive field of the kernel by using gaps when applying the kernel to the input.  By applying dilated convolutions, the author claims it can reduce the degree of signal downsampling, as well as condition on larger  context. Applying the fully connected CRF on the segmentation score map refines the segmentation result and achieves better object localization. As illustrated in Figure~\ref{fig:DeepLabv1}, the downsampled feature map from the fully convolutional network is first upsampled to the original image resolution using bilinear interpolation and then refined by the fully connected CRF to produce the final prediction mask. At  publication time DeepLabv1 achieved the state of the art result of 71.6$\%$ IoU at the PASCAL VOC-2012 semantic image segmentation task. 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv1}
	\caption{ The overall model architecture of DeepLabv1.~\cite{chen2014semantic}}
	\label{fig:DeepLabv1}
\end{figure}
One year later, Chen et al.~\cite{chen2017deeplab} proposed DeepLabv2 by updating DeepLabv1 with 2 major improvements. First, DeepLabv2’s fully convolutional layers used a ResNet CNN as backbone. Second, the author also proposed atrous spatial pyramid pooling (ASPP) to robustly segment objects at multiple scales, illustrated in Figure~\ref{fig:DeepLabv2ASPP}. Specifically, the incoming convolutional feature layers are filtered using multiple parallel dilated convolutional layers with different dilated rates, hence segmenting objects as well as image context at multiple scales. This work established the new state of the art result on PASCAL VOC2012 , achieving 79.7$\%$ IoU.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv2ASPP}
	\caption{ The illustration of ASPP~\cite{chen2017deeplab}}
\label{fig:DeepLabv2ASPP}
\end{figure}
Chen et al. again updated DeepLabv2 to propose a better variant of DeepLab which is DeepLabv3~\cite{chen2017rethinking} by revisiting the use of dilated convolution and removing the use of fully connected CRF. The author experimented with DeepLabv3 with 2 main ideas:
\textbf{ Going Deeper with Atrous Convolution}, illustrated in Figure~\ref{fig:DeepLabv3Cascade} the design is to have  more blocks with atrous convolution in cascade. The dilation introduced in the convolutional kernels makes it easier to capture long range information in the deeper blocks.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3Cascade}
	\caption{  The overview of atrous convolution designed  in cascade in DeepLabv3.~\cite{chen2017rethinking}}
	\label{fig:DeepLabv3Cascade}
\end{figure}
\textbf{The modified Atrous Spatial Pyramid Pooling (ASPP)}, proposed in DeepLabv2 is illustrated in Figure~\ref{fig:DeepLabv3ASPP}. The new ASPP is added with learnable batch normalization, image-level features and 1x1 convolutions. All feature maps produced from multi-parallel dilated convolution with different rates and image-level features are concatenated and processed by the 1x1 convolution, then passed through the final 1x1 convolution to produce final logits.
DeepLabv3 achieved a significant improvement on the PASCAL VOC 2012 dataset with 85.7$\%$ IoU.		
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3ASPP}
	\caption{   The overview of new ASPP in DeepLabv3.~\cite{chen2017rethinking}}
	\label{fig:DeepLabv3ASPP}
\end{figure}

Chen et al. extended DeepLabv3 to release DeepLabv3+~\cite{chen2018encoder} by adapting the system into encoder-decoder semantic segmentation architecture and using atrous convolution layers separable. Figure~\ref{fig:DeepLabv3+} shows the architecture of DeepLabv3+.   The DeepLabv3 network is used as an encoder network with the Xception network as backbone to the fully convolutional layers and still employs the ASPP. Moreover, a new effective decoder network is added to refine the segmentation results especially for large objects. The encoding features are first upsampled using bilinear interpolation and then concatenated with the corresponding and same resolution low-level features from Xception FCNs backbone. Then these concatenated features are convolved and enlarged again to produce the final prediction map. DeepLabv3+ achieved a 3.3$\%$ improvement on the results of DeepLabv3, reaching 89$\%$ IoU on PASCAL VOC 2012 dataset.		
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3+}
	\caption{   The overall encoder-decoder-like semantic segmentation network of DeepLabv3+~\cite{chen2018encoder}}
	\label{fig:DeepLabv3+}
\end{figure}

~\section{Data Augmentation For Image Classification}
\para Recently, data augmentation for images have played a very significant role in the successful training of deep CNN models which typically require a large amount of data. This is a technique of creating more images from information of existing images without changing the meaning of images, hence making the data set more diverse. Applying data augmentation helps the model frequently see more unseen data, consequently tackle the overfitting issue and make the model generalise better. Data augmentation for images is mainly divided into three groups: normal augmentation, neural network based method and augmentation search. 
~\subsection{Normal Augmentation}
\para In normal augmentation, the additional images are generated by using simple mathematical functions that transform various aspects of images such as texture, shape and color. Below we describe some of the most popular data augmentation methods:

~\textbf{Rotation} : The image is rotated clockwise or counter-clockwise by a random angle between 0 to 360 degree. This means the object in the image will be rotated but its shape will not change. Figure \ref{fig:NormalAugmentation}

~\textbf{Flipping} : We can flip the direction of the image either horizontally or vertically. That means the transformed image is horizontally or vertically symmetrical with respect to the original image. Figure \ref{fig:NormalAugmentation}

~\textbf{Shifting}: Shifting augmentation is also known as translation augmentation that moves all pixel values of the image in the left,right,top and bottom direction. In the case that the object in the image moves too far, the image may lose too much information, thus making it impossible to make a correct prediction on its label. Figure \ref{fig:NormalAugmentation}

~\textbf{Crop} : A region of the image is randomly cropped with a determined size. This technique generates new images of smaller size. Figure \ref{fig:NormalAugmentation}

~\textbf{Cutout}~\cite{devries2017improved}: Inspired by the dropout regularization technique~\cite{hinton2012improving}, cutout is the technique that randomly removes a fixed sized region from images and replaces it with random pixel values. It helps the computer vision machine model to see more simulated situations where the object in the image is partially occluded. Moreover, this technique is also relatively similar to Random Erasing~\cite{zhong2017random}. Figure \ref{fig:NormalAugmentation}

~\textbf{Colour Transformation}~\cite{shorten2019survey}: For grayscale images, each pixel contains one intensity value in the range of 0-255 inclusive. For color images, each pixel contains 3 intensity values of color channels represented in a particular color space system such as RGB (Red-Green-Blue), CMY (Cyan-Magenta-Yellow) and HSI (Hue-Saturation-Intensity). To do colour augmentation, four aspects (hue, saturation, brightness and contrast) are manipulated. The most popular methods of colour transformation are histogram equalisation, and adjusting the following: brightness, contrast, white balancing, sharpening and blurring~\cite{mikolajczyk2018data}. Figure \ref{fig:ColorAugmentation}

~\textbf{Noise Injection}~\cite{shorten2019survey}: The image is injected with an amount of noisy pixel value, usually from Gaussian noise in order to help the model to learn more robust features. Figure \ref{fig:NormalAugmentation}
\begin{figure}[h]
	\centering
	\subfloat[Original]{\includegraphics[width=0.3\textwidth]{Original}} 
	\subfloat[Rotated Image]{\includegraphics[width=0.3\textwidth]{Rotation}}
	\subfloat[Horizontal Flipped Image]{\includegraphics[width=0.3\textwidth]{Flip}}
	\qquad
	\subfloat[Top Shifted Image]{\includegraphics[width=0.3\textwidth]{Shift}}
	\subfloat[Cropped Image]{\includegraphics[width=0.2\textwidth]{Crop}}
	\subfloat[Cutout Image]{\includegraphics[width=0.3\textwidth]{Cutout}}
	\qquad
	\subfloat[Noise Injected Image]{\includegraphics[width=0.3\textwidth]{Noise}}
	\caption{ Examples of normal augmentation method on dermatoscopic skin lesion image.} 
	\label{fig:NormalAugmentation} 
\end{figure} 
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{ColorAugmentation}
	\caption{ Examples of colour augmentation~\cite{shorten2019survey}.}
	\label{fig:ColorAugmentation}
\end{figure}
~\subsection{Neural Netwok Based Method}
\para In this method, the new image is generated from a trained neural network and it will preserve the semantic of its label.

~\textbf{Generative Adversarial Networks(GANs)}~\cite{goodfellow2014generative}: The idea of GANs is that having the generative model and the discriminative model, the discriminative model is trained with real data to be able to detect the sample data whether is real or fake. Then, the generative model is trained to pit against the trained discriminative model, that means the generative model releases the sample that is detected as real data by the discriminative model. Figure ~\ref{fig:GAN}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{GAN}
	\caption{Samples are drawn from a generator. The yellow box is the latest version of each sample~\cite{goodfellow2014generative}.}
	\label{fig:GAN}
\end{figure}
~\textbf{Neural Style Transfer}~\cite{gatys2015neural}: This technique is not only known as the creation of artistic images, but is also a very useful technique for image augmentation such that augmented images have the same content as original images but different styles. The idea is to feed two images into two CNNs, one of those contains the content for the new image and the other contains the style. The CNNs will separate and recombine the content and style in order to generate new images. Figure ~\ref{fig:NeuralTransfer}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{NeuralTransfer}
	\caption{The artistic image B is generated by CNNs. The image A is the content image and the small image at bottom-left is style image~\cite{gatys2015neural}.}
	\label{fig:NeuralTransfer}
\end{figure}
~\subsection{Augmentation Search}
\para Manually applying many different random normal augmentation techniques to the training process at the same time makes it hard to figure out which one improves the model's performance. Thus, augmentation search algorithms automatically find an optimal data augmentation policy which determines for a given data set the best set of normal augmentation methods to use and their corresponding best settings.

~\textbf{AutoAugmentation}~\cite{cubuk2019autoaugment}: This method consists of two components: a search algorithm and a search space. The search algorithm uses a reinforcement learning algorithm which finds the best data augmentation policy from the search space. In the search space, a policy consists of many sub-policies. Moreover, each sub-policy has two normal image transformations corresponding with the probability of applying transformations and the magnitude of transformations. 

~\textbf{RandAugmentation}~\cite{cubuk2019randaugment}: AutoAugmentation is computationally expensive due to its focus on finding augmentation policies using a separate search phase performed on proxy tasks which include searching different models and dataset sizes. In contrast, RandAugmentation directly evaluates the impact of the data augmentation on the target model and dataset. This results in a much smaller search space involving the set of available operations, magnitude of all operations and just two hyperparameters (N and M) to tune. 

~\section{Imbalanced Class}
\label{sec:background_imbalance}
	
~\subsection{Image classification}
~\subsubsection{For Supervised learning}
\para Training data often do not have balanced distribution. For example fraud classification from transactional data, fraud transactions are much rarer than non fraud transactions. Another example task in healthcare is cancer detection where there are usually many more healthy samples than cancer samples. Therefore, in the testing phase,  the machine learning model mostly predicts the majority class in the training set rather than the minority class, leading to much lower accuracy for predicting the minority class.   Many methods have been proposed to address class imbalance, which can be grouped into three categories: data-level, algorithm-level and hybrid approaches~\cite{johnson2019survey}.

~\textbf{Data-level Approach}: Before feeding the data into the model during training, the dataset is resampled to create a balanced distribution across classes. This randomly reduces the number of majority class samples and  randomly increases the sampling of the minority class. However there are some downsides of these techniques, according to ~\cite{johnson2019survey} under-sampling the majority class might substantially reduce the  amount of information from the eliminated data.  Over-sampling will increase training time and may cause the model to over-fit. To overcome these downsides, several advanced sampling methods have been proposed in the literature. For under-sampling, in  ~\cite{mani2003knn,kubat1997addressing,barandela2004imbalanced}, intelligent methods are used to efficiently select which majority class samples are eliminated. For oversampling in~\cite{chawla2002smote,han2005borderline,bunkhumpornpat2009safe}, intelligent methods are used to create new artificial minority class samples from existing minority class samples.

~\textbf{Algorithm-level Approach}: Instead of resampling the data distribution, this method modifies the model’s algorithm to give more emphasis on the minority class and can be divided into 3 approaches~\cite{johnson2019survey}: new loss function, cost-sensitive learning and threshold moving. Mean False Error~\cite{wang2016training}, Focal Loss~\cite{lin2017focal}, Weighted Cross Entrpy Loss~\cite{phan2017dnn} are new loss functions that reduce the effect of majority class on the loss. In cost-sensitive learning~\cite{wang2018predicting,khan2017cost,zhang2016training}the model learns from the classification cost matrix, that means each class is assigned different costs. Lastly, in the threshold moving technique~\cite{krawczyk2015cost,chen2006decision,yu2016odoc}, the idea is to adjust the decision threshold to reduce bias on easy samples, in other words, make more correct predictions on hard samples.

~\textbf{Hybrid-level Approach}: There are several hybrid methods~\cite{he2009learning,dong2018imbalanced}that combine both of the above approaches that firstly resamples data distribution and then applies algorithmic approaches such as cost-sensitive learning.

~\subsubsection{For Semi-Supervised Learning}

\para All of the above methods which alleviate skewed data distribution only works for supervised learning where we know the labelled data distribution. It is really challenging to use a semi-supervised learning approach where the distribution of the unlabelled data is unknown.

\textbf{Suppressed Consistency Loss}: For SSL perturbation based methods,  Minsung ~\cite{hyun2020class} has proposed an algorithm level method which is Suppressed Consistency Loss (SLC). In  the imbalanced class learning environment, the decision boundary is more likely to move into the low-density areas of the minor class  with consistent regularization that causes the model to misclassify the minor class. Therefore, SLC will suppress the consistency loss of minor classes which in turn tends to push the decision boundary against the low-density areas.

~\subsection{Semantic segmentation}
\para While classification suffers from class imbalance at the whole image grain, semantic segmentation suffers from the same problem at the pixel grain. Especially in binary medical image segmentation, the number of background class pixels is often much larger foreground class pixels. The methods to deal with class imbalance in semantic segmentation are also divided into 2 main groups:  data level and algorithmic level approaches. 

\textbf{Data level}: It is difficult to use oversampling or undersampling methods developed for image classification for semantic segmentation. According to~\cite{taghanaki2019combo}, it would be meaningless to undersample an image by removing some major class pixels/voxels because it would remove a lot of information from the image.  For  patch-based segmentation approaches, there are several existing works~\cite{ciresan2012deep,milletari2017hough} that  use the patch selection algorithm to balance the number of patches from major and minor classes. 

\textbf{Algorithmic level}: Algorithmic approaches are more commonly used to address class imbalance for segmentation tasks. These methods include Weighted Cross Entropy Loss~\cite{phan2017dnn}, Focal Loss~\cite{lin2017focal}, Dice Loss~\cite{sudre2017generalised} which is built from Dice Coefficient metric and aims to maximize the similarity of two images , Tversky Loss~\cite{salehi2017tversky} which modifies Dice Coefficient metric in a way that weigh False Negative more than False Positive and pre-compute weight map for the ground truth in UNet~\cite{ronneberger2015u}.

To our knowledge there are no studies that mainly focus on dealing with class imbalance in the context of semi supervised semantic segmentation. Therefore, we address this gap in the literature.	 		


==> Paper arxiv/Section/competing_interest.tex <==
~\section*{Declaration of Competing Interest}
\para The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work reported in this paper.

==> Paper arxiv/Section/conclusion.tex <==
\section{Conclusion}
\para In this study, we identified an important gap in existing literature: class imbalance in the context of semi-supervised learning for medical images. This is an important problem to study since medical image datasets often have skewed distributions and missing positive disease diagnosis can have fatal consequences. We address this gap by proposing a new consistency loss function called Adaptive Blended Consistency Loss (ABCL). To demonstrate the effectiveness of ABCL, we applied it to the perturbation based semi-supervised learning algorithm UDA. ABCL extends standard consistency loss by generating a new blended target class distribution from the mix of original and augmented sample’s class distribution. Extensive experiments showed ABCL consistently outperforms alternative approaches designed to address the class imbalance problem. Our proposed ABCL method was able to improve the performance of UDA baseline from 0.59 to 0.67 UAR, outperform methods that address the class imbalance problem for labelled data (between 0.51 and 0.59 UAR) and for unlabelled data (0.61 UAR) on the imbalanced skin cancer dataset. On the imbalanced retinal fundus glaucoma dataset, combining with Weighted Cross Entropy loss, ABCL achieved 0.67 UAR as compared to 0.57 to its nearest rival. The results on both datasets show that ABCL can be combined with methods designed to address class imbalance for supervised learning to further boost performance on semi-supervised learning. As future work we plan to evaluate ABCL on other medical imaging tasks, such as semi-supervised semantic segmentation.








==> Paper arxiv/Section/experiment_setup.tex <==
\section{Experiment Setup}
\subsection{Dataset}
\para We evaluate our proposed methodology on skin cancer and retinal fundus glaucoma datasets:

\begin{itemize}
	\item HAM10000 ~\citep{tschandl2018ham10000} (main dataset) : contains 10015 RGB dermatoscopic skin lesions images of size (450, 600) multiclass, divided into 7 classes: Pigmented Bowen’s (AKIEC), Basal Cell Carcinoma (BCC), Pigmented Benign Keratoses (BKL), Dermatofibroma (DF), Melanoma (MEL), Nevus (NV), Vascula (VASC).
	\item REFUGE Challenge~\citep{orlando2020refuge} (supporting dataset) : contains 1200 RGB retinal fundus glaucoma images of various sizes. Each image is assigned a binary label of glaucoma or non-glaucoma.
	
\end{itemize}
~\autoref{fig:classificationimage} shows example images for each class. As is shown in ~\autoref{tab:classificationdistribution}, the class distributions of both datasets are highly imbalanced.
\begin{figure}
	\centering
	\subfloat[]{\includegraphics[width=1\textwidth]{SkinImage.png}} 
	\newline
	\subfloat[]{\includegraphics[width=1\textwidth]{REFUGE.png}} 
	\caption{Example images of the dermatoscopic skin lesions and retinal fundus glaucoma dataset for each class.}
	\label{fig:classificationimage}
\end{figure}
\begin{table}
	\begin{subtable}{1\textwidth}
		\scriptsize
		\begin{tabular}{| l | l | l | l | l | l | l | l | l | l |}
			\hline
			\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Skin cancer dataset}}}  &\textbf{MEL} &\textbf{NV} &\textbf{BCC} &\textbf{AKIEC} &\textbf{BKL} &\textbf{DF} &\textbf{VASC} &\textbf{Total} \\
			\cline{2-9}
			& 1113  & 6705  & 514  & 327  & 1099  & 115  & 142 & 10015 \\
			\cline{2-9}
			& 0.11 & 0.67 & 0.06 & 0.03 & 0.11 & 0.01 & 0.01 & 1 \\
			\hline
			
		\end{tabular}
	\end{subtable}
	\bigskip
	\newline
	\vspace*{0.5 cm}
	\begin{subtable}{1\textwidth}
		\scriptsize
		\begin{tabular}{| l | l | l | l |}
			\hline
			\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Retinal fundus glaucoma dataset}}}  & \textbf{Glaucoma} &\textbf{Non-Glaucoma)} &\textbf{Total}  \\
			\cline{2-4}
			& 120  & 1080 & 1200  \\
			\cline{2-4}
			& 0.1 & 0.9 & 1 \\
			\hline
		\end{tabular}
	\end{subtable}
	\caption{The class distribution of 2 experimental classification datasets. Both datasets are very imbalanced. The range of class frequencies frequency is (0.67,0.01) for skin cancer dataset and (0.9,0.1) for retinal fundus glaucoma dataset.}
	\label{tab:classificationdistribution}
\end{table}

We split the datasets as follows: 70$\%$ training images, 20$\%$ test images and 10$\%$ validation images. We use the validation dataset to decide when to perform early stopping when training the model. All the results reported in the paper are from the test dataset. Notably, the unlabelled training dataset is deliberately larger than the labelled training dataset in order to simulate the  problem we described earlier. We ensure the class distribution across each of the data splits are the same. 

\subsection{Data processing}
\para For the HAM10000 dataset, the model is trained with the original image size of (450, 600), in contrast, images of the REFUGE challenge dataset are resized to (512,512). All images of both datasets have their color normalised. In particular, the red and blue color channel will be normalised based on the green color channel. The formula is described as follows: 	
\begin{equation*} 
       R = R * ( \frac{G_{mean}}{R_{mean}}) ; 	B = B *(\frac{G_{mean}}{B_{mean}})      
\end{equation*}


\subsection{Evaluation metrics}
\para Due to the class imbalance in the testing dataset, the model usually performs really well on the major classes and much worse on the minor classes. By looking at the overall accuracy, we might be tempted to say that the model has good performance, but actually it only achieves high accuracy on major classes. However, minor class accuracy is really important, especially for medical image analysis since often the samples with disease belong to the minor class. Hence, the Skin Lesion Analysis towards Melanoma Detection (ISIC 2018)~\citep{gutman2016skin} competition used an evaluation metric that gives equal weight to all classes (called unweighted average recall (UAR)) to rank the performance of the different models. Therefore, we also use UAR to measure our model’s performance across all classes in a fair way. In addition we report results using the G-mean and average Area Under the ROC curve (AUC) metric since they are also commonly used in other studies involving classification of imbalanced classes~\citep{kaur2019systematic}.   	

\subsection{Model training}

\para All models were trained for 200 epochs with the static learning rate of $10^{-4}$. To implement early stopping we use the model that gave the best validation UAR for measuring results on the test set. Furthermore, the Stochastic Gradient Descent (SGD) optimizer with momentum 0.9 and weight decay 5 x $10^{-4}$ was used. During training we use a batch size of 30 samples consisting of 8 labelled samples and 22 unlabelled samples.

\subsection{Data Augmentation}
\label{sec:data_augmentation}
\para Strong data augmentation via RandAugmentation~\citep{cubuk2019randaugment} is a key component of the UDA method, and the authors show that it can significantly improve the sample efficiency by encouraging consistency on a diverse set of augmented examples. However, experiments presented in ~\autoref{sec:weak_strong} show ABCL performs poorly when strong data augmentation is used. We attribute the poor performance of ABCL in the presence of strong data augmentation to increased distance between the augmented and unaugmented examples in embedding space. ABCL assumes in cases 3 and 4 of ~\autoref{tab:4 cases} (one of the predictions belongs to a major class and the other belongs to a minor class), it is more likely the actual class is the minor class. However, when using strong data augmentation, the augmented major class sample may be moved far away from the original example in feature space. As a consequence, there is a risk the augmented sample may be predicted to be a different class. That is, samples belonging to the major classes are more likely to be predicted wrongly since the strong augmentation can make very significant changes to the appearance of the images. Consequently, the main assumption behind ABCL is violated when strong data augmentation is used. Hence, we use weak data augmentation for both labelled and unlabelled samples which include random horizontal flips, rotations (between 0 and 180 degree), erasing~\citep{zhong2017random} (a random proportion (0.02-0.33) of input image will be erased) and color augmentation (jitter brightness, saturation and contrast with a random value in range of 0.9 to 1.1). 




\subsection{Algorithms used in experimental study}

\para \textbf{\emph{UDA baseline}}. The original UDA method is implemented to obtain the baseline method. This baseline is not designed to handle class imbalance. All other methods implemented modify this baseline UDA method. As default we use weak data augmentation for all algorithms implemented in this paper including UDA baseline. However in~\autoref{sec:weak_strong} we show an experiment where we compare the performance of strong versus weak data augmentation for UDA and UDA+ABCL. The results show that ABCL with weak data augmentation is able to outperform UDA using strong data augmentation. This shows that benefits of using ABCL outweigh the performance loss from using weak data augmentation. 

\textbf{\emph{Sampling based method for the labelled dataset}}. We will resample the skewed labelled dataset by using the intelligent oversampling method SMOTE~\citep{chawla2002smote} and random undersampling.

\textbf{\emph{Weighted Cross Entropy Loss (WeightedCE)}}. This is an extension of the Cross Entropy loss function which weights the loss of each class based on a given set of weights. The objective of WeightedCE is to give higher loss for the minor class and lower loss for the major class. Intuitively, it helps the model reduce the effect of the major class. We define the set of class weights as follows:
\begin{itemize}
	\item Class frequency :  [0.11,0.67,0.06,0.03,0.11,0.01,0.01] for the HAM10000 dataset and [0.1,0.9] for the REFUGE dataset
	\item weight = 1 - Class frequency 
\end{itemize}

\textbf{\emph{Focal Loss~\citep{lin2017focal}}}. This loss function is used for supervised learning to reduce the effect of the \qq{easy samples} (samples belonging to the major class). The default $\gamma$ value used was 1 because we found this value for $\gamma$ gave the best UAR result when we did a hyperparameter search.

\textbf{\emph{Consistency loss suppression (SCL)~\citep{hyun2020class}}}. This is the state-of-the-art SSL method used to address class skew that suppresses the consistency loss when the minor class is predicted. We implemented this approach on top of UDA.  The default $\beta$ value used was 0.8 because we found this value gave the best UAR result when we did a hyperparameter search.

\textbf{\emph{Adaptive Blended Consistency Loss (ABCL)}}. This is our method for addressing the class imbalance problem for SSL implemented on top of UDA. Our new method has only one hyperparameter: the class imbalance compensation factor $\gamma$. The default $\gamma$ value used was 0.4 because we found this value gave the best overall result when considering UAR and the individual recall results for each class. 

\textbf{\emph{UDA-WeightedCE-SCL and UDA-WeightedCE-ABCL}}. This method combines supervised and unsupervised class imbalance methods. We combine WeightedCE with SCL and ABCL. We chose WeightedCE since we found WeightedCE performs the best among all the supervised class imbalance methods.



==> Paper arxiv/Section/highlights.tex <==

\begin{itemize}
	\item We identify the importance of handling class imbalance for semi-supervised classification of medical images. In contrast, no existing work explicitly addresses this problem for medical images.
	\item A new method Adaptive Blended Consistency Loss is proposed as a replacement for the consistency loss of perturbation based semi-supervised learning (SSL) algorithms in order to tackle the class imbalance problem in SSL.
	\item Our Adaptive Blended Consistency Loss outperformed the standard consistency loss and other existing methods designed for addressing the class imbalance problem in both supervised and semi-supervised learning. 
\end{itemize}

==> Paper arxiv/Section/introduction.tex <==
\section{Introduction}
\para Computer-aided diagnosis is an important field of research, as well-written algorithms can improve diagnostic efficiency and reduce the chance of misdiagnosis. For example, at the early stages tumors or lesions might be very small and easy for a radiologist to miss, but by using an algorithm to automatically highlight such instances the number of false negatives can be reduced. Recently, many supervised machine learning methods, especially those using convolutional neural networks (CNNs) have achieved promising results in medical image classification, an important component of computer-aided diagnosis ~\citep{rezvantalab2018dermatologist,han2018classification,bi2017automatic,hekler2019superior,iizuka2020deep,ausawalaithong2018automatic,rajpurkar2017chexnet}. However supervised learning requires a large number of fully labelled medical images. In the real world, annotating medical images is typically very time-consuming, especially when the consensus of multiple experts is required.  Fortunately, in many practical situations there are often many unlabelled images available that can be leveraged to boost model accuracy. Semi-supervised learning (SSL) ~\citep{chapelle2009semi}
 makes use of a small amount of labelled and a large amount of unlabelled data to  train machine learning models. The goal of SSL is to learn patterns from unlabelled data to enhance the accuracy of a model that is trained using a small amount of labelled data. There are several variants of SSL dealing with medical image classification tasks which have achieved promising results such as Categorical Generative Adversarial Networks~\citep{springenberg2015unsupervised}, Denoising Adversarial AutoEncoders~\citep{creswell2018denoising}, Dual-path Semi-supervised Conditional Generative Adversarial Networks~\citep{yang2019dscgans}, and the MeanTeacher with Label Propagation algorithm~\citep{su2019local}. Recently researchers have found perturbation based methods give the best performance~\citep{xie2019unsupervised,tarvainen2017mean,laine2016temporal,miyato2018virtual,berthelot2019mixmatch}. Hence in this study we will focus on perturbation based methods. Most perturbation based algorithms augment unlabelled data and then apply a consistency loss to make the predicted class distribution from the original and augmented (perturbed) unlabelled samples similar.
 
 There are several techniques based on this approach which recently achieved state of the art results, mostly on various classification tasks, such as Temporal Ensembling~\citep{laine2016temporal}, Mean Teacher~\citep{tarvainen2017mean}, Virtual Adversarial Training~\citep{miyato2018virtual}, Unsupervised Data Augmentation (UDA)~\citep{xie2019unsupervised} and MixMatch~\citep{berthelot2019mixmatch}.
 
Medical image datasets often have a very skewed data distribution, usually due to a large number of negative disease cases versus a small number of positive disease cases. It is critically important to address this class imbalance problem since failure to address this problem can lead to false negatives for the minor class (the disease-positive case) which can have potentially fatal consequences. This motivates us to study techniques for dealing with skewed data in SSL.	 	

Almost all existing approaches for handling skewed data distributions are only for  labelled datasets including: various oversampling or undersampling approaches ~\citep{mani2003knn,kubat1997addressing,barandela2004imbalanced,chawla2002smote,han2005borderline,bunkhumpornpat2009safe}; modified loss functions~\citep{wang2016training,lin2017focal,phan2017dnn}; cost sensitive learning~\citep{wang2018predicting,khan2017cost,zhang2016training}; decision threshold moving~\citep{krawczyk2015cost,chen2006decision,yu2016odoc}. In our case we would like to develop effective methods for addressing the skewed class distribution of unlabelled data for SSL. 

We focus our study on modifying the consistency loss (loss on unlabelled data) on one of the best performing recent SSL methods, Unsupervised Data Augmentation (UDA)~\citep{xie2019unsupervised}. Although our study is focused on UDA, our proposed method can be applied to any perturbation based SSL which uses the consistency loss such as Temporal Ensembling~\citep{laine2016temporal}, Mean Teacher~\citep{tarvainen2017mean} and Virtual Adversarial Training~\citep{miyato2018virtual}. The standard consistency loss (CL) used in UDA has two shortcomings: 1) it degrades the classification performance of the minor classes, and 2) it always sets the target as the original sample instead of a blend of the augmented and original sample. Hence, we propose the Adaptive Blended Consistency Loss (ABCL) method which tackles both shortcomings of standard consistency loss by generating a target class distribution which is a blend of the original and augmented class distributions. The blended target class distribution skews towards either the original or augmented sample depending on which predicted the minor class.

To our knowledge the only existing work that addresses the class distribution skew problem for SSL perturbation based methods is the Suppressed Consistency Loss (SCL) method~\citep{hyun2020class}. Their observation is that for class imbalanced datasets, the training is likely to move the decision boundary into the low-density areas of the minor class which will in turn cause the model to misclassify minor class samples. Therefore, SCL suppresses the consistency loss of minor classes which will help move the decision boundary away from the low-density areas that the minor classes occupy. However SCL, like the standard consistency loss of UDA, also sets its target as the original sample instead of a blend of the augmented and original samples. This will in general favor the major class since the models are more likely to predict the major class as a result of the bias inherent in the unbalanced dataset itself. In contrast, our ABCL uses a blended target class distribution that skews towards either the original or augmented sample depending on which predicts the minor class.

We have conducted an extensive experimental study on a skin cancer HAM10000 dataset~\citep{tschandl2018ham10000} and a retinal fundus glaucoma REFUGE dataset~\citep{orlando2020refuge}. Our experiments show that when our ABCL method is used to replace the consistency loss of UDA, the unweighted average recall (UAR) on HAM10000 increases from 0.59 to 0.67.  Furthermore,  ABCL also significantly outperformed the state-of-the-art SCL method for the skin cancer dataset. For the retinal fundus glaucoma dataset, ABCL significantly outperformed SCL, increasing UAR from 0.57 to 0.67. These results show that ABCL is able to improve performance of SSL for different datasets.


This paper makes the following key contributions:
\begin{itemize}
	\item We identify the importance of handling class imbalance for semi-supervised classification of medical images. In contrast, no existing work explicitly addresses this problem for medical images.
	\item We propose the Adaptive Blended Consistency Loss (ABCL) as a replacement for the consistency loss of perturbation based SSL algorithms such as UDA in order to tackle the class imbalance problem in SSL.
	\item We conduct extensive experiments on two different datasets to demonstrate the advantages of ABCL over standard consistency loss and other existing methods designed for addressing the class imbalance problem in both supervised learning and SSL. 
\end{itemize}




==> Paper arxiv/Section/keywords.tex <==
\para Semi supervised learning; Medical Imaging; Class Imbalance

==> Paper arxiv/Section/methodology.tex <==
\section{Material and methods}
~\subsection{Semi-supervised learning architecture}
\para We base our research on perturbation based SSL methods since all state of the art SSL methods ~\citep{xie2019unsupervised,tarvainen2017mean,laine2016temporal,miyato2018virtual,berthelot2019mixmatch} use this approach.
The solution we developed for this paper can be applied to any perturbation based SSL that uses the consistency loss. To simplify our analysis we will focus on a particular perturbation based SSL called the Unsupervised Data Augmentation~\citep{xie2019unsupervised} (UDA) method. UDA is one of the best performing recent SSL methods.~\autoref{fig:UDA} shows a diagram of how UDA works. The model is trained using two losses: a supervised loss (cross-entropy loss) and an unsupervised loss (consistency loss). The aim of consistency loss is to enforce the consistency of two prediction distributions. The key idea of UDA is to use optimal data augmentation on unlabelled samples to increase the effectiveness of the consistency loss. To obtain optimal data augmentation they applied an algorithm called RandAugmentation~\citep{cubuk2019randaugment} on the labelled dataset.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{UDA.jpg}
	\caption{ The architecture used by the  Unsupervised Data Augmentation (UDA) ~\citep{xie2019unsupervised} perturbation SSL method. In the diagram M is the shared CNN model used for classifying both the labelled and unlabelled images.
	}
	\label{fig:UDA}
\end{figure}
The total loss for the UDA architecture consists of two terms (see ~\autoref{fig:UDA}): supervised loss for labelled data and consistency loss for unlabelled data. The loss formula can be summarized as follows:
\begin{equation}
	\label{eqn:uda_equation}
	L =  L_{S}( p_{\theta}(y|l) ) + L_{con}( p_{\theta}(y|u) , p_{\theta}(y|\hat{u}) )
\end{equation}

Where $L_{S}$ is a supervised cross entropy loss function that takes input as the predicted probability distribution $p_{\theta}(y|l)$ of $y$ for a  labelled sample $l$ produced by the model $M$ with parameters $\theta$. $L_{con}$ is a consistency loss function that uses the Kullback-Leibler divergence to steer the predicted class distribution of the augmented unlabelled image $\hat{u}$ towards the target predicted class distribution of the original unlabelled image $u$.

A key assumption of perturbation based methods such as UDA is the smoothness assumption. Under the smoothness assumption, two data points  that are close in the input space should have the same label. That means, an unlabelled sample that is close to a labelled example will have the label information propagated to the unlabelled sample. Another important property of the smoothness assumption is that the original input and the augmented input should be close to each other in the embedded space and hence should be assigned the same label. This idea is captured by the consistency loss $L_{con}$ which ensures the model produces the same predicted probabilities from both the original and augmented input, leading to the model being robust to noise. 	

There have been various existing approaches~\citep{mani2003knn,kubat1997addressing,barandela2004imbalanced,chawla2002smote,han2005borderline,bunkhumpornpat2009safe,wang2016training,lin2017focal,phan2017dnn,wang2018predicting,khan2017cost,zhang2016training,krawczyk2015cost,chen2006decision,yu2016odoc} to tackle class imbalance for the supervised learning problem. These approaches are complementary to our solutions since they work on improving supervised loss while ours works to improve the unsupervised loss component of the overall loss. The unsupervised loss is particularly important since the number of unlabelled examples is typically much larger than labelled examples. As shown in ~\autoref{fig:UDA},  UDA uses the consistency loss to exploit the information from the unlabelled loss by making the class distribution of the augmented unlabelled data match the original unlabelled data. Hence to alleviate the class imbalance problem in UDA, we focus on modifying UDA’s consistency loss (shown in ~\autoref{eqn:uda_equation}). In particular, UDA’s consistency loss is replaced by our new novel loss function, Adaptive Blended Consistency Loss (ABCL). Hence the total loss is reformulated with ABCL replacing the unsupervised term: 
 
\begin{equation}
	L =  L_{S}( p_{\theta}(y|l) ) + ABCL( p_{\theta}(y|u) , p_{\theta}(y|\hat{u}) )
\end{equation}


\subsection{Issues with existing consistency loss formulations}
\label{sec:problems_cl_scl}
\para In this section, we analyse problems with standard consistency loss (CL) in UDA~\citep{xie2019unsupervised} and the state-of-the-art suppressed consistency loss (SCL)~\citep{hyun2020class} when training on datasets with imbalanced class distributions. The problems will be analysed in the context of the original sample’s prediction (OSP) and augmented sample’s prediction (ASP) which represent the probability distributions $ p_{\theta}(y|u)$ and  $p_{\theta}(y|\hat{u})$ respectively in ~\autoref{eqn:uda_equation}

~\autoref{fig:Normal CL} illustrates how CL and SCL works. In UDA, the CL is a function that sets the OSP as the target for ASP. That is the CL always pushes the class distribution of ASP towards the class distribution of OSP. The idea behind SCL is to suppress the minor class‘s consistency loss to move the decision boundary such that it passes through a low-density region of the latent space. In practical terms, SCL suppresses the CL when the OSP is the minor class and applies the CL when the OSP is the major class. Like CL, SCL uses the OSP’s class distribution as the target irrespective of whether OSP and ASP class distributions belong to the major or minor class.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{NormalCL.jpg}
	\caption{ An illustration showing how CL and SCL works. Note that the target class distribution is always the class distribution for OSP. In addition, SCL down-weights the loss if the predicted class of OSP is the minor class.}
	\label{fig:Normal CL}
\end{figure}

Both standard CL and SCL have two shortcomings. Firstly they are both biased towards targeting the major class in the presence of imbalanced training data. Secondly they do not target a blend of OSP and ASP but instead always target OSP only, and thus do not exploit the augmented example to improve the model's behaviour for the original example.

~\textbf{~\emph{Shortcoming 1: CL and SLC are more likely to target the major class}}. When in doubt the model will more often predict the major class since the model is trained on labelled data which is skewed towards major class samples. Consequently, samples of the minor class are more likely to be mispredicted as the major class than vice versa. In particular, when the original sample is incorrectly predicted as major class and the augmented sample is correctly predicted as minor class, the CL and SCL erroneously encourages the model to predict the sample as major class. As a result, the model’s performance will degrade for minor class samples.

~\textbf{~\emph{Shortcoming 2: CL and SLC do not target a blend of OSP and ASP but instead always targets OSP only}}. Targeting a blend of OSP and ASP reduces the harmful effects of targeting OSP only when OSP predicts the wrong class. Unlike existing methods, we do not make the assumption that the model’s prediction for the original sample is more accurate than for the augmented sample. Instead we set the target as a blend of OSP and ASP to potentially average out some of the harmful effects of a wrong OSP prediction. This is in some ways similar to the benefit of ensembling the prediction of multiple models to minimize prediction error and the established technique of test-time data augmentation~\citep{krizhevsky2012imagenet}.

The shortcomings mentioned above are all centered around what we should set as the target distribution for the CL as a function of OSP and ASP. Hence, to provide a more detailed analysis of the desired target class distribution we divide the analysis into four separate cases depending on whether major or minor classes were predicted by the OSP and ASP.
\begin{table}
	\footnotesize
	\begin{tabular}{|m{0.7cm}|m{1.7cm}|m{1.7cm}|m{1.7cm} |m{1.7cm} |m{1.7cm}|}
		\hline
		\textbf{Case} & \textbf{OSP} & \textbf{ASP} & \textbf{CL target} & \textbf{SCL target} & \textbf{ABCL target} \\
		\hline
		
		1 & Major class & Major class & OSP (major class) &OSP (major class) & Near the middle between OSP and ASP \\
		\hline
		
		2 & Minor class &Minor class &OSP (minor class) &OSP (minor class) & Near the middle between OSP and ASP \\
		\hline
		
		3 & Major class & Minor class & OSP (major class) & OSP (major class) & Closer towards ASP \\
		\hline
		
		4 & Minor class & Major class & OSP (minor class) & OSP (minor class) & Closer towards OSP \\
		\hline
	\end{tabular}
	\caption{The analysis of the target class distribution of CL (standard consistency loss), SCL (suppressed consistency loss), and our ABCL (adaptive blended consistency loss) for 4 prediction cases. ~\autoref{fig:4 case illustration} gives a diagrammatic illustration of the 4 cases.}
	\label{tab:4 cases}
\end{table}
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{4caseillustration.jpg}
	\caption{ An illustration of the target class distribution of CL, SCL and ABCL for the 4 cases shown in ~\autoref{tab:4 cases}.}
	\label{fig:4 case illustration}
\end{figure}
See ~\autoref{tab:4 cases} and ~\autoref{fig:4 case illustration} for an illustration of the 4 different OSP and ASP cases. In cases 1 and 2, OSP and ASP are in agreement. Unlike CL and SCL, we forgo the assumption that the OSP is in any way more valid than the ASP. As a result, we posit that it may be better to move the desired target class distribution to be a blend of OSP and ASP instead of just to OSP. This is because we would like the target to contain information in the predictions of both OSP and ASP. In case 3 CL and SCL may unintentionally encourage the bias towards the major class to be stronger since it is moving the desired target class distribution towards the major class although there is no consensus between the two predictions. There is already a natural tendency to predict the major class, a bias which is induced by the dataset skew. CL/SCL does nothing to counteract this bias as it does not consider the frequencies of the predicted classes. Case 3 presents an opportunity to counteract this bias, as the model has already indicated via the ASP that the minor class is likely correct since it made that prediction despite its natural tendency to predict the major class. Unfortunately, using CL/SCL in this situation is likely to encourage the model to mispredict the minor class sample as the major class. It would be preferable to instead move the desired target class distribution towards ASP, thus counteracting the dataset bias. In case 4, OSP is the minor class, so there is no bias towards the major class and so both CL and SCL do a good job of rewarding the minor class prediction in this case.

\subsection{Adaptive Blended Consistency Loss (ABCL)}
\label{sec:abcl}
\para To address the drawbacks of CL and SCL, the desired target class distribution for the consistency loss should be adaptively adjusted to be somewhere between OSP and ASP depending on which of the 4 cases in ~\autoref{tab:4 cases} and ~\autoref{fig:4 case illustration} has occurred. In cases 1 and 2, OSP and ASP both are either the major or minor class. In this case the desired target class distribution should be in the middle of OSP and ASP. In case 3 and 4, to discourage the bias towards predicting the major class, the desired target distribution should be closer to the minor class depending on whether OSP or ASP is the minor class. 

We proposed a new consistency loss function called Adaptive Blended Consistency Loss (ABCL) which captures the desirable properties listed above.~\autoref{fig:ABCL}  illustrates how it works. ABCL uses the following loss function to generate a new target class distribution which is a blend of OSP and ASP.
\begin{equation}
	 ABCL (z,\hat{z} ) = L_{con}(z_{blended},z) + L_{con}(z_{blended},\hat{z})
\end{equation}
\begin{equation}
	z= p_{\theta}(y|u) ; \hat{z} = p_{\theta}(y|\hat{u})  
\end{equation}
$L_{con}$ is the Kullback-Leibler divergence between the blended target probability distribution $z_{blended}$ and either OSP ($z$) or ASP ($\hat{z}$). Hence ABCL pulls both the original and augmented predictions towards the target distribution. For a model with parameters $\theta$, $p_{\theta}(y|u)$ and $p_{\theta}(y|\hat{u})$ denote the predicted class probability distribution for an original unlabelled example $u$ and its augmented version $\hat{u}$ respectively. The gradient of the loss is not be back-propagated through $z_{blended}$ during parameter optimisation.

The blended target class distribution $z_{blended}$ is defined as follows:
\begin{equation}
	z_{blended} =   (1 - k)*z+ k*\hat{z}
\end{equation}
Where $k$ is the weighting value [0,1] that determines the proportion to which the blended target moves towards OSP versus ASP. When $k$ equals 0, the target will become OSP meaning ABCL will become the same as CL. On the other hand, as $k$ approaches 1, the target approaches ASP. $k$ is calculated based on predicted class frequencies with respect to the training dataset using the following formula:
\begin{equation}
	\label{eqn:determine k}
	k= max(0, min(\gamma*(N_{original}-N_{augmented} ) + 0.5 ,1))
\end{equation}
$N_{original}$ and $N_{augmented}$ are the class frequencies of the predicted class (class with the highest predicted probability) for the OSP and ASP respectively. $\gamma \in$ (0, 1] is the class imbalance compensation strength that controls how strong the new blended target class distribution skews towards either OSP or ASP.
The value of $k$ can be interpreted as follows:
\begin{itemize}
	\item When the OSP is the minor class and the ASP is the major class (case 4 in ~\autoref{tab:4 cases} and ~\autoref{fig:4 case illustration}), the value of $N_{original}$ will be smaller than the value of $N_{augmented}$ so the value of $k$ will be smaller than 0.5. This indicates that the new blended target class distribution will skew towards the minor class side (OSP).
	\item When the OSP is the major class and the ASP is the minor class (case 3 in ~\autoref{tab:4 cases} and ~\autoref{fig:4 case illustration}), the value of $N_{original}$ will be larger than the value of $N_{augmented}$ so the value of $k$ will be larger than 0.5. This indicates that the new blended target distribution will skew towards the minor class side (ASP).
	\item When OSP and ASP both are the major class or both are the minor class (cases 1 and 2 in ~\autoref{tab:4 cases} and ~\autoref{fig:4 case illustration}), the value of $N_{original}$ and $N_{augmented}$ are similar, so the value of $k$ will be around 0.5. In this case OSP and ASP contribute equally to the blended target distribution.
\end{itemize}

~\textbf{~\emph{Class imbalance compensation strength $\gamma$}}. In ABCL (~\autoref{eqn:determine k}), the $\gamma$ term is used to control how strongly the new blended target distribution is pushed towards either OSP or ASP. As $\gamma$ approaches 0, the impact of $N_{original} - N_{augmented}$ on the value of $k$ will be smaller, and $k$ will therefore be close to 0.5. This indicates that the new blended target class distribution will skew only slightly to either OSP or ASP. On the other hand, as $\gamma$ approaches 1, the impact that $N_{original} - N_{augmented}$ has on $k$ will be bigger. This indicates that the new blended target class distribution will skew strongly to either the OSP or ASP. When $\gamma$ is set to a high value, ABCL approaches the standard CL in the case that $N_{augmented} >> N_{original}$, since $z_{blended} \approx z$. This corresponds to CL, where OSP is wholly responsible for defining the target of the unsupervised loss term.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{ABCL.png}
	\caption{Diagram showing  how ABCL works. The target distribution is blended more towards the minor class, although it still retains some of OSP’s distribution.}
	\label{fig:ABCL}
\end{figure}





==> Paper arxiv/Section/problem_definition.tex <==

\para As a result of our thorough literature review, we found there is no prior work  addressing the class imbalance problem in semi-supervised learning of medical images for either classification or segmentation. Therefore in this thesis we will  address the class imbalance problem for both semi-supervised medical image classification and segmentation. 

Semi-supervised learning (SSL) for medical images is of practical importance. Large numbers of labelled training images are necessary for training highly accurate deep learning classification and segmentation models. However, it is costly and time-consuming for medical experts to manually annotate the required number of images at either image-level or pixel-level. Hence, semi-supervised learning is an ideal method to tackle this obstacle. It only requires a small portion of all scanned images to be labelled and automatically exploits statistical patterns from the rest.  Medical image datasets often contain studies that involve imbalanced datasets which the model trained on often favour the majority image class (usually negative cases), such as for the HAM10000 skin cancer dataset~\cite{tschandl2018ham10000} where the  majority of the images are classified as benign versus a small number of malignant images, for ChestX-ray14 dataset~\cite{wang2017chestx} where the majority of the images are for healthy lungs versus unhealthy lungs, or for the  Nerve Ultrasound segmentation dataset~\cite{nervesegmentation} where the number of background pixels is heavily larger than foreground pixels. Hence in this study we address the class imbalance issue for semi-supervised classification and segmentation of medical images. 


As stated earlier our problem of class imbalance in semi-supervised learning for medical images has not been explored directly in the past. There are still several studies of SSL medical images on skewed data distributions~\cite{yi2018unsupervised,creswell2018denoising,nie2018asdnet,zheng2019semi}  but they  are not focused on  addressing the class imbalance problem. There has also been work addressing the class imbalance problem for \textit{supervised} learning---such as resampling  ~\cite{mani2003knn,kubat1997addressing,barandela2004imbalanced,chawla2002smote,han2005borderline,bunkhumpornpat2009safe,ciresan2012deep,milletari2017hough}, loss function ~\cite{lin2017focal,phan2017dnn}, region-based loss~\cite{sudre2017generalised,salehi2017tversky}, cost-sensitive learning ~\cite{wang2018predicting,khan2017cost,zhang2016training}, threshold moving ~\cite{krawczyk2015cost,chen2006decision,yu2016odoc} and using a pre-compute weight map for ground truth~\cite{ronneberger2015u}---but none of these works study SSL. We found one study~\cite{hyun2020class} that proposed  a new loss function for addressing the class imbalance issue for SSL. However, the authors conduct their experiments on standard image datasets and as such the efficacy of their proposed approach remains unproven on medical image datasets where minimising the number of false negative predictions is extremely important. Furthermore they artificially made their datasets imbalanced by introducing synthetic skew into the class distribution. In contrast, our study will use a medical image dataset which contains a real skewed class distribution.



\para More formally we define our problem as follows. Given a set of $n$ labelled training examples $L = \{l_{1}, l_{2}, ...l_{n}\}$ and a set of $m$ unlabelled  training examples $U = \{u_{1}, u_{2}, ...u_{m} \} $, with $m >> n$. The class distribution of labels in $L$ and $U$ are highly skewed, so both class distributions have low entropy. We further assume that samples in both $L$ and $U$ are drawn from the same population, and hence the class distributions of $L$ and $U$ are similar.

For the image classification task, the aim is to train a model using both $L$ and $U$ such that the model achieves high average recall for all classes (the standard metric for judging the success of models on class imbalanced datasets). Hence we aim to maximize the unweighted average recall ( UAR) metric on a test data set of $z$ examples $T = {t_{1}, t_{2}, ...t_{z}}$. UAR is defined as follows:

\begin{equation*}
	\text{UAR} = \frac{\sum\limits_{C=1}^C Recall_{C}}{C}
\end{equation*}

For the image segmentation task, the aim is to train a model using both $L$ and $U$ such that the model achieves high dice coefficient metric for minor class ona test data set of $z$ examples $T = {t_{1}, t_{2}, ...t_{z}}$. Dice coefficient is defined as follows:

\begin{equation*}
	\text{Dice} = \frac{2 * TP}{2 * TP + FP + FN}
\end{equation*}

Further details of the UAR and Dice coefficient can be found in~\ref{sec:evaluation_metrics}.

We assume that $T$ has the same class distribution as $L$ and $U$.  By using the UAR  metric, we evaluate the model based on the contribution of all classes equally rather than favoring the major classes. Furthermore,  it will make sure the minor classes which are really important for us (normally ones with disease) get an equal share of the error metric.  Similarly the Dice Coefficient fairly measures performance of every class regardless of class distribution skew.

\para ~\textbf{\emph{Justification for assuming labelled and unlabelled data have the same class distribution}}: Our new loss function mainly depends on the information of the predicted class‘s frequency of unlabelled data. We can not measure the class distribution of the unlabelled dataset. Therefore, in our study, we assume that the class distribution of the unlabelled dataset is the same as the labelled dataset. This assumption is also supported by statistical theory. That is, the data distribution of a population can be represented by the data distribution of a uniform random sample from the population. In our problem, the labelled dataset is a sample taken from the population. We can use its class distribution to represent the population. Hence, it is reasonable to assume the unlabelled data has the same class distribution as the labelled data for a sufficiently large number of samples. 






==> Paper arxiv/Section/related.tex <==
~\section{Semi-Supervised Learning}
\label{sec:ssl}
\para Our focus is on intrinsically semi-supervised methods, a subclass of inductive semi supervised learning. In order to make use of unlabelled data, these methods often follow smoothness and low-density assumptions. The low-density assumption states that the decision boundary should pass through low-density areas in the data space. The smoothness assumption states that if two data points are close, it should have the same predicted label~\cite{chapelle2009semi}. Based on the assumption, the perturbation based method increases the robustness of the model by utilizing noise on unlabelled data. That means the original input and the input perturbed with noise should both produce the same predicted label. There are several techniques based on  this approach which recently achieved state of the art results, mostly on various classification tasks, such as Temporal Ensembling~\cite{laine2016temporal}, Mean Teacher~\cite{tarvainen2017mean}and Virtual Adversarial Training~\cite{miyato2018virtual}.

~\textbf{$\prod$-MODEL}~\cite{laine2016temporal}: Inspired by ensemble learning, the idea is to encourage the consistency of a model to two of its outputs $z$ and $\tilde{z}$, which is produced from the same input by applying different dropout and data augmentation conditions, over each batch training.  Figure~\ref{fig:Temporal} shows the learning framework. The model is learned from two losses, the supervised loss on $z$ prediction of only labelled inputs by using the cross entropy loss function and mean squared loss between the $z$ and $\tilde{z}$. On CIFAR-10 with only 4000 labels, the $\prod$-MODEL achieved an error rate of 12.36$\%$.

~\textbf{Temporal Ensembling}: This technique is built on top of the $\prod$-MODEL with the difference being the model only produces one output $z$ and the prediction $\tilde{z}$ is based on the model’s output in the previous epoch. The learning framework has shown in the same figure of $\prod$-MODEL, Figure~\ref{fig:Temporal}. After every training epoch, the model’s output $z$ is accumulated into an ensemble of outputs $Z$ by updating $Z$ ← $\alpha$$Z$ + (1$-$ $\alpha$)$z$ and calculating $\tilde{z}$ by dividing $Z$ by factor (1$-$$\alpha^t$).
By only producing one output at the time, the Temporal Ensembling learning method is faster than $\prod$-MODEL. Moreover, the output $\tilde{z}$ calculated in the previous epoch can be expected to have less noise than the one in $\prod$-MODEL. The slightly better result is reported on 4000 labels of CIFAR-10 with 12.16$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{Temporal}
	\caption{~\cite{laine2016temporal} Learning framework of $\prod$-MODEL and Temporal Ensembling method.}
	\label{fig:Temporal}
\end{figure}

~\textbf{Mean Teacher}: This technique consists of the dual student and teacher models which produce $z$ and $\tilde{z}$ prediction from all inputs X by applying two types of stochastic noise. Figure~\ref{fig:MeanTeacher} illustrates the learning framework. The weights $\theta$ of the student model is updated by the supervised loss on only labelled data of student’s output $z$  and the consistency loss which is the distance between student’s output $z$  and teacher output $\tilde{z}$ from the entire input. Whereas, the teacher’s weight $\theta$’ is updated by the exponential moving average of the student's weight over each batch training, which computed as follows: $\theta'_{t}$ = $\alpha\theta'_{t-1}$  + (1 $-$ $\alpha)\theta_{t}$. On 4000 labels of CIFAR-10 and trained on ResNet, the Mean Teacher achieved the state of the art result with 6.28$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MeanTeacher}
	\caption{~\cite{tarvainen2017mean} Learning framework of MeanTeacher method.}
	\label{fig:MeanTeacher}
\end{figure}

~\textbf{Virtual Adversarial Training}~\cite{miyato2018virtual}: Most perturbation based methods apply stochastic augmentation to the input. However, in this approach, the authors directly applied small directional noise to the corresponding input which makes the model‘s prediction change the most, also known as adversarial example ~\cite{goodfellow2014explaining}. Basically, the method is inspired by Adversarial Training~\cite{goodfellow2014explaining} which uses the following loss function: 
\begin{equation}
	L_{adv}(x_{l},\theta) := D[q(y|x_{l}),p(y|x_{l} + r_{adv},\theta)]
\end{equation}
\begin{equation}
\text{where }r_{adv}:=\operatorname*{arg\,max}_{r;||r||\leq\epsilon} D[q(y|x_{l}),p(y|x_{l} + r,\theta)]
\end{equation}
The goal of the loss function is to minimize the divergence between the true distribution of output label $q(y|x_{l})$ and the model’s output distribution $p(y|x_{l} + r_{adv},\theta)$ by applying adversarial noise $r_{adv}$ to inputs $x_{l}$. However, the adversarial training only works well on supervised tasks. To transfer to the semi-supervised task, the loss function is reformulated as:
\begin{equation}
	L(x_{*},\theta) := D[p(y|x_{*},\hat{\theta}),p(y|x_{*} + r_{adv},\theta)]
\end{equation}
\begin{equation}
\text{where }r_{adv}:=\operatorname*{arg\,max}_{r;||r||_{2}\leq\epsilon} D[p(y|x_{*},\hat{\theta}),p(y|x_{*} + r)]
\end{equation}
Where $x_{*}$ is either unlabelled $x_{u}$ or labelled $x_{l}$. Indeed, we can not obtain $q(y|x_{u})$, therefore the authors  proposed the term called virtual labels which replaces $q(y|x_{*})$ with its current output $p(y|x_{*},\hat{\theta})$. This is the reason for the use of the terms “virtual” on all of the techniques reported by the paper including virtual adversarial training, virtual adversarial noise. On 4000 labels of CIFAR-10, the Virtual Adversarial Training achieved the state of the art result with 10.55$\%$ error rate.

~\textbf{Unsupervised Data Augmentation}~\cite{xie2019unsupervised}: the authors found applying advanced data augmentation on unlabelled samples could effectively make the model more invariant to noisy input in the semi-supervised learning approach. Instead of applying only some normal data augmentations such as flip, rotation in Temporal Ensembling, Mean Teacher or virtual adversarial noise in Virtual Adversarial Training, they used an auto augmentation method called ~\textbf{RandAugmentation}~\cite{cubuk2019randaugment} to find policies and magnitudes of chosen transformations which yield the best performance on labelled samples and then apply these to unlabelled samples. As a result, on CIFAR 10 with 4000 labels, this approach achieved a 5.29$\%$ error rate which is near the state of the art result for supervised learning approach. 

~\textbf{MixMatch}~\cite{berthelot2019mixmatch}: This approach does not fully belong to perturbation based method because it just utilizes the idea of perturbation based semi-supervised method as a part of the algorithm. MixMatch unifies current dominant approaches such as perturbation based semi-supervised learning methods discussed above, entropy minimization which encourages the model to make low entropy prediction on unlabelled samples and ~\textbf{MixUp}~\cite{zhang2017mixup}, a technique that combines samples for training. Moreover, these approaches are combined to generate a new set of labelled data $X$’ and unlabelled data $U$’ with predicted labels. In more detail, firstly, apply data augmentation on a batch of labelled samples $X$ and unlabelled samples $U$, to create augmented batches $\hat{X}$ and $\hat{U}$. Then, construct the predicted labels for augmented $\hat{U}$ by applying a Sharpening function to reduce the  entropy of the average model’s predictions on augmented $\hat{U}$ Figure ~\ref{fig:MixMatch}. Next, to prepare for the MixUp step, shuffle $\hat{X}$ and $\hat{U}$ with predicted labels to create set $W$. After that, apply the MixUp function on $\hat{U}$ and a part of $W$ samples, $\hat{X}$ and the rest of $W$ samples to produce a new set of labelled data $X$’ and unlabelled data $U$’. Finally, the authors just used the standard semi-supervised learning loss framework which uses the cross entropy loss function for MixUp $X$’ model’s prediction of labelled data, L2 loss for MixUp $U$’ model’s predicted outputs on unlabelled data. With 4000 labels on CIFAR 10, this technique achieved the state of the art result of 4.95$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MixMatch}
	\caption{~\cite{berthelot2019mixmatch} Diagram of the label guessing process in MixMatch.}
	\label{fig:MixMatch}
\end{figure}

Another subcategory of intrinsically semi-supervised learning is generative models. The primary characteristic of this method is to generate new unlabelled data for classification.

~\textbf{Categorical Generative Adversarial Networks}~\cite{springenberg2015unsupervised}: The idea is to build on top of ~\textbf{GANs}~\cite{goodfellow2014generative} which consists of the discriminator and generative functions and only work on unsupervised tasks. To deal with semi-supervised tasks, the authors made an extension to the discriminator so that classifies K class for all samples from the labelled dataset and discriminates real versus fake samples from the generator. Intuitively, the job of the generator is changed from “generate samples that belong to the real dataset” to “generate samples that belong to the K class dataset”.  Additionally, cross entropy loss term is also added to penalize the error of discriminator’s prediction on real data and corresponding labels. As a result, on standard 4000 labels CIFAR, the network achieved a 19.58$\%$ error rate.

~\section{Semi supervised learning in semantic segmentation}
\para In this section, we review several popular semi-supervised semantic segmentation frameworks which combine small amounts of pixel-level labeled data with large amounts of data that are either weakly labeled or not labelled. Weak labels include bounding boxes or image-level labels.
~\subsection{Weakly- and Semi-Supervised Learning of a Deep Convolutional Network for Semantic Image Segmentation (2015)}
\para Papandreou et al.~\cite{papandreou2015weakly} propose a semi-supervised framework for semantic segmentation by using DeepLab as a segmentation network and proposing Expectation-Maximization (EM) algorithm to estimate the segmentation mask from weakly labeled data. The total loss has two components, illustrated in Figure~\ref{fig:SSLDeepLab}: one on strongly labeled data is from the prediction map produced by DeepLab network with its pixel-level annotations; another loss on weakly labeled data is from the prediction map produced by DeepLab network with its estimated pixel-level map which is generated from the EM algorithm. They conducted their experiments using the PASCAL VOC 2012 dataset, with 1400 strong labels and 9000 weak labels (image-level labels) which is generated by summarizing the pixel-level annotations. The proposed method achieved 66$\%$ IoU.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLDeepLab}
	\caption{DeepLab model training methodology using a combination of pixel-level (strong labels) and image-level (weak labels) annotations.~\cite{papandreou2015weakly}}
	\label{fig:SSLDeepLab}
\end{figure}

~\subsection{Revisiting Dilated Convolution: A Simple Approach for Weakly and Semi -Supervised Semantic Segmentation (2018)}
\para Wei et al.~\cite{wei2018revisiting} proposed the semi-supervised semantic segmentation method that uses the dilated convolutions for object localization. The training framework includes two modules using shared fully convolutional networks(FCNs) as the segmentation network backbone, shown in Figure~\ref{fig:SSLRevisiting}: 

The first module works on image-level labelled data. The proposed augmented classification network that has aVGG 16 backbone with multi-dilated convolutional (MDC) blocks  produces the dense localization map. The dense localization map is then further processed to generate the segmentation mask. This segmentation mask serves as supervision in the loss function with the segmentation mask produced by FCNs and the ground truth image-level label.

The second module is the normal supervised FCNs segmentation which employs pixel-level labeled data. The loss from two modules is combined to perform the semi-supervised learning. This method achieved 67.6 IoU on the PASCAL VOC 2012 dataset with 1400 strong labels and 9000 weak labels.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLRevisiting}
	\caption{ Diagram illustrating the semi-supervised semantic segmentation method proposed by Wei et al.~\cite{wei2018revisiting}  }
	\label{fig:SSLRevisiting}
\end{figure}

~\subsection{Adversarial Learning for Semi-Supervised Semantic Segmentation (2018)}
\label{sec:ssl_adv3}
\para Exploiting the success of GANs~\cite{goodfellow2014generative}, Hung et al.~\cite{hung2018adversarial} proposed the adversarial learning for semi-supervised semantic segmentation. The framework contains two networks, segmentation network which is DeepLabv2 and discriminator network, shown in Figure~\ref{fig:SSLAdversarial}. Instead of classifying an image as real or fake, the author designed the FCN discriminator to distinguish between the predicted probability  maps from the ground truth segmentation maps. In the semi-supervised training process, the method uses strong labeled data and unlabeled data which is a new feature in this study. When using strong labeled data, the segmentation network is trained using two loss functions: Cross-entropy loss ($L_{ce}$) on the segmentation ground truth and adversarial loss ($L_{adv}$) to fool the discriminator. When using unlabeled data, the segmentation network is trained with Cross entropy semi-supervised loss ($L_{semi}$). Specifically, the predicted segmentation map of the unlabeled image produced by the segmentation network is passed through the discriminator network to obtain the confidence map. Then, in the context of self-training, this confidence map serves as a target for the previous segmentation prediction in the $L_{semi}$ loss. Notably,  the discriminator network is only trained with the strongly labeled data. The study achieved 69.5$\%$ IoU on PASCAL VOC 2012 dataset using 1400 strong labeled images and 9000 unlabeled images.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLAdversarial}
	\caption{ Diagram illustrating the  Adversarial semi-supervised semantic segmentation framework~\cite{hung2018adversarial}  }
	\label{fig:SSLAdversarial}
\end{figure}

\subsection{Semi-Supervised Semantic Segmentation with High and Low-level Consistency (2019)}
\label{sec:ssl_adv4}
\para Mittal et al.~\cite{mittal2019semi} proposed a semi-supervised segmentation framework that contains two branches which are illustrated on Figure~\ref{fig:SSLs4GANMLMT}. Their method is called the Semi-Supervised Semantic Segmentation GAN-based network (s4GAN)  which improves the low-level details in the segmentation output using semi-supervised multi-label classification via the MeanTeacher approach.  s4GAN exploits class-level information to remove false-positive predictions from the segmentation map. The s4GAN branch consists of a DeepLabv2 segmentation network and a discriminator network. The segmentation network  acts as a generator to produce the segmentation maps from input images and is trained together with a discriminator network  responsible for distinguishing the ground truth segmentation maps from the generated ones. The segmentation network is trained with three loss functions: the Cross Entropy loss applied on the pixel level  labels; the feature matching loss and self-training loss applied on the unlabeled data. The discriminator network is trained with the original GAN loss: learns to differentiate between the real ground truth maps and the prediction segmentation maps of unlabeled data. The MLMT branch is the semi-supervised classification MeanTeacher network~\cite{tarvainen2017mean} which is backed by ResNet101 and works on both image-level labeled data and unlabeled data. Notably, the s4GAN and mean teacher network branches are trained separately. 

The output of the mean teacher network is the predicted classification score for all classes. This is then used to refine the predicted segmentation maps from s4GAN to produce the final prediction segmentation mask. The prediction segmentation mask for a particular class is removed from the maps if its classification score is less than the predefined threshold.This method achieved 71.4$\%$ IoU  on the PASCAL VOC data set using 1400 strongly labeled data samples and 9000 unlabeled data samples.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLs4GANMLMT}
	\caption{ Diagram illustrating the semi-supervised semantic segmentation method proposed by Mittal et al.~\cite{mittal2019semi} called the s4GAN + Multi-label MeanTeacher classifier.  }
	\label{fig:SSLs4GANMLMT}
\end{figure}

~\subsection{Semi-Supervised Semantic Segmentation with Cross-Consistency Training (2020)}
~\label{sec:ssl_cs5}
Ouali et al.~\cite{ouali2020semi} presented a cross-consistency based training method for semi-supervised semantic segmentation. The idea is to use the encoder-decoder as the segmentation architecture and perturbation-based approach, discussed in Section~\ref{sec:ssl}, for semi-supervised learning. Specifically, there is one encoder and one main decoder and multiple auxiliary decoders, as shown in Figure~\ref{fig:SSLMultiDecoder}. The encoder and main decoder is trained using supervised Cross Entropy loss with pixel level targets. For the unlabeled examples, the encoder and all auxiliary decoders are trained using unsupervised loss by applying a consistency loss between the main decoder predictions and all auxiliary decoder predictions which are produced from different types of noise applied to the inputs of the auxiliary decoders. Notably, the unsupervised loss is not back-propagated through the main-decoder. The study established a new state of the result of 69.4$\%$ IoU on the PASCAL VOC 2012 dataset.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLMultiDecoder}
	\caption{ Semi-Supervised Encoder-Decoder Semantic Segmentation with Cross-Consistency Training~\cite{ouali2020semi}.}
	\label{fig:SSLMultiDecoder}
\end{figure}

~\subsection{Semi-supervised semantic segmentation needs strong, varied perturbations (2020)}
~\label{sec:ssl_cs6}
\para French et al.~\cite{french2020semi} proposed a perturbation based semi-supervised semantic segmentation method that uses the MeanTeacher framework~\cite{tarvainen2017mean}. The method used strong varied perturbations such as CutOut, CutMix. The segmentation network used is DeepLabv2 and DenseUnet trained on 2 losses: the supervised Cross Entropy loss on pixel-level labeled data and unsupervised consistency loss on unlabelled data. Specifically for the unlabelled data, the unsupervised consistency loss enforces the consistency between the target, which is the prediction segmentation maps of the Teacher network on the original image, and the predicted segmentation maps of the Student network. The input to the student network is strongly augmented data using methods such as CutOut and CutMix. With this simple semi-supervised framework, the study achieved 67.6$\%$ IoU on the PASCAL VOC 2012.

~\section{CNNs For Medical Image Classification}
\para Medical imaging has played a crucial diagnostic role in modern medicine. The common types of medical image can be divided as follows: Ultrasound which is the  safest method for the patient’s health and is generated by using sound waves; X-Ray which is the oldest technology and generated by using electromagnetic radiation; CT (Computer tomography) which builds the 3D image based on X-Rays; and MRI ( Magnetic Resonance Imaging) which is generated by using a strong magnetic field and radio waves~\ref{fig:MedicalImage}. Besides the four common imaging types listed above, there is another type of medical image used for skin lesions that generate dermoscopy images using skin surface microscopy. In addition, medical image is obtained to visualize the information of the internal human body in order to support pathologists, radiologists or clinicians to make a diagnosis about the disease. The final diagnosis of a patient’s health should be made by doctors based on combined evidence from various processes and scans of the patient. Manually analysing medical images for multiple patients is a laborious, repetitive task and error prone task for doctors. Therefore automated diagnosis would help doctors work more efficiently. One of the most common underlying technologies of these systems is deep learning which leverages a substantial amount of medical imaging data. Deep convolutional neural networks (CNNs) are the dominant technique for this task. There are many applications of using deep CNNs in medical imaging tasks including tumor segmentation, cancer detection, cancer classification, image guided therapy, medical image annotation, and image retrieval~\cite{anwar2018medical}. To confine the scope in this section we only describe the application and research in the area of cancer classification using supervised CNNs. The result and objective of each study can vary depending on such factors as quantity and quality of the dataset, number of classes to classify and CNN network architecture used.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MedicalImage}
	\caption{ Medical imaging modalities~\cite{anwar2018medical}.}
	\label{fig:MedicalImage}
\end{figure}
~\subsection{Skin Cancer Classification}
\para Han et.al.~\cite{han2018classification} worked on classifying 12 skin diseases which include basal cell carcinoma, squamous cell carcinoma, intraepithelial carcinoma, actinic keratosis, seborrheic keratosis, malignant melanoma, melanocytic nevus, lentigo, pyogenic granuloma, hemangioma, dermatofibroma and wart. They used the ResNet152 CNN model~\cite{he2016deep} to train on roughly 19000 clinical images from the Asan, MED-Note and Alas dataset. They tested on the Asan test dataset which achieved 0.91, 86.4, 85.5 for AUC, Sensitivity, Specificity respectively. When using the Edinburgh test dataset, they achieved 0.89, 85.1, 81.3 for AUC, Sensitivity, Specificity respectively.

Amirreza et.al.~\cite{rezvantalab2018dermatologist} experimented on dermoscopy images (~\cite{tschandl2018ham10000}HAM10000: 10015, ~\cite{mendoncca2013ph}PH2 : 120) which includes 8 types of skin diseases: melanoma, melanocytic nevi, basal cell carcinoma, benign keratosis, actinic keratosis and intraepithelial carcinoma, dermatofibroma, vascular lesions, and atypical nevi. They tried to use 4 different CNN models pre-trained on ImageNet including:  Google’s Inception v3~\cite{szegedy2016rethinking}, InceptionResNetv2~\cite{szegedy2017inception}, ResNet152~\cite{he2016deep}, and DenseNet201~\cite{huang2017densely}. As a result, they reported that the DenseNet201 model achieved the best accuracy among the 4 models in terms of micro and macro averaged precision (89.01$\%$ - 85.24$\%$), F1 - Score (89.01$\%$ - 85.13$\%$), and ROC AUC (98.79$\%$ - 98.16$\%$), even outperforming expert dermatologists’s performance.

Bi et.al.~\cite{bi2017automatic} worked on the problem of classifying the 3 skin diseases of melanoma, seborrheic keratosis and nevus on 3600 dermoscopy images including 1600 from the ISIC Archive dataset~\cite{gutman2016skin}. The final CNN classification model is assembled from 3 separated classification models such that one outputs 3 skin disease classes and the two others output the binary classification of melanoma versus others and seborrheic keratosis versus others. The reported result on AUC is 91.5$\%$.

Achim et.al.~\cite{hekler2019superior} involved a combination of the deep learning and skin cancer experts to build a superior skin cancer classification algorithm. Firstly, a ResNet CNN model is trained on 11,444 dermoscopic images, obtained from HAM10000 and ISIC Archive, to classify 5 skin diseases. Then both the CNNs trained model and dermatologists of German university hospitals will classify 300 test biopsy-verified images. Finally, a gradient boosting method is used to produce a new classifier from the confident outputs of the CNN model and the dermatologists. This method achieved accuracy, sensitivity and specificity results of  (82.95$\%$, 89$\%$, 84$\%$), compared to standalone dermatologists test results of  (42.94$\%$, 66$\%$, 62$\%$) and CNN model results of  (81.59$\%$, 86.1$\%$, 89.2$\%$).

~\subsection{Digital Pathology Classification}
\para Digital pathology is a field that uses computer-based technology to manage information generated specimens on slides. With the evolution of Whole Slide Images (WSI) technology which transforms the specimens on glass slides into digital high resolution images, known as histopathology image, digital pathology brings a new way to potentially help pathologist’s diagnosis more efficiently by using deep learning. However, one of the challenges in applying deep learning, specifically deep CNNs on WSI, is the very high dimensionality of the input, for example millions of pixels. Therefore, besides configuration of the model, the successful deep CNNs on pathology task also heavily depend on WSI image preprocessing.

Stomach and colon cancers are common cancers that cause high numbers of deaths worldwide, and in a 2018 report, there are 782,685 and 551,269 deaths due to stomach and colon cancer respectively. In addition, new research by Osamu et.al.~\cite{iizuka2020deep} used deep learning techniques to perform histopathological classification of stomach and colon cancer. There were three classes : adenocarcinoma, adenoma and non-neoplastic. The dataset consists of 4,128 and 4,036 whole slide images (WSIs) of the stomach and colon respectively collected from Hiroshima University and Haradoi Hospital. CNN Google’s Inception v3 model is trained on millions of patches extracted from WSIs to classify the three classes above. Then a max-pooling approach and a recurrent neural network (RNN) is used to predict the final label for the particular WSI by aggregating all it’s patch predictions.The model achieved the following AUC results, 0.97 and 0.99 for gastric adenocarcinoma and adenoma, 0.96 and 0.99 for colonic adenocarcinoma and adenoma.

Lung carcinoma is also a dangerous cancer that causes death to humans and the process of histologic pattern analysis in lung carcinoma is a very significant process in lung cancer diagnoses. Jason et.al.~\cite{wei2019pathologist} collected 422 WSIs from the Dartmouth-Hitchcock Medical Center in Lebanon.They used deep CNN Resnet architecture to classify histologic patterns on resected lung adenocarcinoma WSIs. The CNN model classifies patches extracted from the given WSI into histologic subtype patterns. Then, a heuristic is used to infer predominant and minor histologic patterns for the given WSI by aggregating its patch predictions. At the testing phase combined with experts, this method achieved a kappa score of 0.525 and an agreement of 66.6$\%$ with three pathologists, slightly higher than the inter-pathologist kappa score of 0.485 and an agreement of 62.7$\%$.

Another health problem which also receives high attention from researchers is the breast cancer. Kun et.al.~\cite{fan2019deep} applied the pipeline framework, which uses the highlight from a heat-map to classify whether the WSI contains breast cancer metastases on the Camelyon-16 grand challenge dataset. Firstly, the deep CNN Google’s Inception v3 architecture is trained to classify patches extracted from WSIs as tumor or normal. Then each WSI is slided into many patches, and fed into the trained CNN to build the tumor probability heat-map. After that, a Support Vector Machine classifier is trained on WSIs’s heat-map to finally produce the label for the entire WSI. As a result,this system achieved 90.23$\%$ of AUCs.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{BreastCancer}
	\caption{~\cite{fan2019deep}The framework of cancer metastases detection.}
	\label{fig:BreastCancer}
\end{figure}
~\subsection{X-ray Classification}
\para X-ray image is one of the most frequently used medical imaging modality. It is used for diagnosing patients because it is cheap and quick to obtain. Therefore using deep learning to diagnose disease from X-rays is well motivated.

Worawate et.al.~\cite{ausawalaithong2018automatic} performed binary classification on the presence of lung cancer. They used a pre- trained deep CNN DenseNet architecture to firstly retrain on the ChestX-ray14 dataset (112,120 non-cancer chest X-ray images) and then fine-tuned on the JSRT dataset (247 chest X-ray images that have 100 lung cancer) in order to alleviate the problem of small samples in the target classification task. The proposed method yielded 74.43$\%$ of mean accuracy, 74.96$\%$ mean specificity and 74.68$\%$ mean sensitivity.

 Lung pneumonia is a cause of death in humans. In 2017 a group from Stanford University~\cite{rajpurkar2017chexnet}proposed CheXNets, which uses a DenseNet 121 trained on ChestX-ray14 dataset to classify X-ray images into 14 disease classes of lung pneumonia. In the testing phase, the model achieved 0.435 F1 score which outperformed the F1 score of 0.387 achieved from averaging 4 scores from radiologists.
 
 \section{Semi-Supervised Learning In Medical Imaging Classification}
 \para In the real world, doing annotations for medical imaging usually is very time consuming for the doctors, especially when the diagnosis of multiple doctors needs to be averaged. Therefore, it is practical to apply semi-supervised learning on medical imaging classification that alleviate the problem of small amounts of labelled medical images and high availability of unlabelled medical images.
 
 For skin cancer classification on ISBI and PH2 dataset, Xin et. al.~\cite{yi2018unsupervised} used ~\textbf{Categorical Generative Adversarial} networks~\cite{springenberg2015unsupervised} in a semi supervised manner to solve two tasks, the first one is to classify the real image into melanoma or benign class, the second one is to generate synthetic images that assist the training. With only 140 labelled images, the method yielded an average precision of 0.424.
 
 In another study of skin cancer classification, Antonia et.al.~\cite{creswell2018denoising} proposed a SSL approach called ~\textbf{Denoising Adversarial AutoEncoder} that combines the Adversarial Net and AutoEncoder Net. Unlabelled samples are utilized in the generative and decoder part to help the model learn the representation of skin cancer such as color, shape and texture. labelled samples are encoded by the encoder and then are classified as either benign or malignant by the discriminator. Due to the heavy class imbalance (0.9,0.1), the classification loss is weighted for each class. On the ISIC dataset with 5000 labelled samples, the SSL approach achieved 0.82 for sensitivity and 0.85 for specificity.
 
 In the study of nucleus classification task, Hai et. al.~\cite{su2019local} integrated the current state of the art SSL approach of MeanTeacher~\cite{tarvainen2017mean} and the graph, which is generated by the Label Propagation algorithm~\cite{zhou2004learning}, that transfers the label information from labelled samples to unlabelled samples. Then the student model is learnt from classification loss, consistency loss and Siames loss which is based on the graph. On the MoNuseg dataset of 22462 nuclei including 4 types of nucleus Epithelial, Inflammatory, Fibroblast and Miscellaneous, the model yielded 75.79 for F1 score using only 10$\%$ of the labelled samples from the dataset.
 
 Moreover, Wenkai et. al.~\cite{yang2019dscgans} combined Semi-supervised Generative Adversarial Nets sGANs, Conditional Generative Adversarial Nets cGANs and Semi Supervised Support Vector Machine S3VM to construct the model called DScGANs (dual-path semi-supervised conditional generative adversarial networks) to solve the thyroid nodule classification task. Notably, the DScGANs is trained under conditional constraint Domain Knowledge (DK) which is acquired from the processed patches called OS, which has 225 pixel value for nodule region and 0 pixel value for non-nodule region, based on consultation with experienced radiologists. The role of DK can be summarized as follows: provide the auxiliary information to help the generator improve image quality; make the connection between information of labelled data and unlabelled data; and acts as a condition to constrain the S3VM to classify the lesion image as benign or malignant. With only 35$\%$ labelled samples from 3090 ultrasonography thyroid nodule lesion images, the proposed method achieved 90.5$\%$ for accuracy and 91.4$\%$ for AUC.
 
 \section{Semi supervised learning in medical semantic segmentation}
 \para For semantic segmentation of medical images, obtaining pixel-level annotation of 2D images or 3D volumes by medical experts is costly and time-consuming, leading  there to be much more unlabeled data compared to labelled data. Therefore, semi-supervised learning is a promising learning framework for medical images that leverages a limited amount of pixel-level labeled data and a large amount of unlabeled data.  There has been many semi supervised frameworks proposed for semantic segmentation of medical images. They can be  grouped into 2 broad types: adversarial training~\cite{nie2018asdnet,zhang2017deep,zheng2019semi,li2020shape}  and consistency training~\cite{bortsova2019semi,li2018semi,yu2019uncertainty}. These methods use the same basic methodology as those used for general semantic segmentation methods that were described  in Sections~\ref{sec:ssl_adv3},~\ref{sec:ssl_adv4} for adversarial training and Sections~\ref{sec:ssl_cs5},~\ref{sec:ssl_cs6} for consistency training.
 


==> Paper arxiv/Section/results.tex <==
\section{Experiment Results}
~\subsection{Results for the  skin cancer (HAM10000) dataset}
\label{sec:skin_resullt}
~\autoref{tab:overall_results} shows the test set results (UAR as the main metric and G-mean, average AUC as supporting metrics) comparing our ABCL with other methods for the HAM10000 dataset. All semi-supervised methods are based on the UDA method. Our ABCL achieved the highest UAR, G-mean and average AUC values of 0.67, 0.62 and 0.95 respectively among all experimented methods. Existing class imbalance methods designed for labelled data (Sampling and Focal) performed worse than the baseline UDA method for the UAR and G-mean metric meaning they were not effective at addressing the class imbalance problem in SSL. This is because these methods can only make a small contribution to overall model quality since they can only be applied to the labelled data which in SSL is just a small portion of the total dataset. 
On the other hand, class imbalance methods designed for unlabelled data (SCL and our ABCL) outperformed the baseline UDA for the UAR and G-mean metrics meaning these methods are more effective than methods which are only applicable to labelled data. This is because these methods modify the consistency loss which is used for the unlabelled data (occupies a larger proportion of all data for SSL) .

When WeightedCE was used with ABCL and SCL, the UAR performance was boosted from 0.67 to 0.68 and from 0.61 to 0.65 respectively. This can be explained by the fact  addressing class imbalance for the labelled data helps the model produce lower bias of the major class for the pseudo target distribution in the unsupervised consistency loss. 
Additionally, although the SCL outperformed the baseline UDA, its performance was still worse than our ABCL in all experiments that involved both methods. This is because as discussed in ~\autoref{sec:problems_cl_scl}, SCL has the two problems of bias towards major class and ignoring the augmented sample prediction when determining the target class distribution.

To further understand the performance of ABCL against the rival methods, we also reported the test set recall of each class in ~\autoref{tab:recall_classes}. This allows us to see how the major and minor classes contribute to the UAR. ABCL performed the best among all methods for almost all of the minor classes (MEL,BCC,BKL,VASC) and performed worse than most methods for the major class NV. This result shows ABCL is doing what it was designed to do, namely, it alleviates the bias towards the major class unlike CL and SCL.

\begin{table}
	\begin{tabular}{l c c c}
		\toprule
		\textbf{Algorithms} & \textbf{UAR} & \textbf{G-mean}   & \textbf{Average AUC}\\
		\midrule
		Supervised learning & 0.75 & 0.71 & 0.98\\
	
		UDA baseline & 0.59 & 0.56 & 0.91\\
	
		UDA-Sampling & 0.51 & 0.44 & 0.89\\ 
	
		UDA-WeightedCE & 0.59 & 0.55 & 0.92\\
		
		UDA-Focal  & 0.55 & 0.50 & 0.92\\
		
		UDA-SCL & 0.61 & 0.58 & 0.92\\
		
		UDA-WeightedCE-SCL & 0.65 & 0.64 & 0.94 \\
		UDA-ABCL(ours) & 0.67& 0.62 & 0.95\\
		UDA-WeightedCE-ABCL(ours) & \textbf{0.68} & \textbf{0.66} & \textbf{0.96} \\
		\bottomrule
	\end{tabular}
	\caption{ Test set results of supervised learning, UDA baseline and various methods designed for handling class imbalance on top of UDA for the HAM10000 dataset. The results in bold show the best result for each column among the unsupervised methods.}
	\label{tab:overall_results}
\end{table}


\begin{table}
	\scriptsize
	\begin{tabular}{m{2cm} m{0.7cm} m{0.7cm} m{0.7cm} m{0.9cm} m{0.7cm} m{0.7cm} m{0.7cm} | m{0.7cm}}
		\toprule
		\textbf{Algorithms} &\textbf{MEL (0.11)} &\textbf{NV (0.67)} &\textbf{BCC (0.06)} &\textbf{AKIEC (0.03)} &\textbf{BKL (0.11)} &\textbf{DF (0.01)} &\textbf{VASC (0.01)} &\textbf{UAR} \\
		\midrule
		UDA baseline & 0.43 & 0.93 & 0.81 & 0.35 & 0.55 & 0.50 & 0.56 & 0.59 \\
		
		UDA-Sampling & 0.44 & 0.84 & 0.69 & 0.52 & 0.53 & 0.36 & 0.12 & 0.51 \\ 
		
		UDA-Weighted Loss & 0.39 & 0.94 & \textbf{0.83} & 0.40 & 0.53 & 0.41 & 0.59 & 0.59 \\ 
		
		UDA-Focal & 0.34 &\textbf{0.96} & 0.81 & 0.32 & 0.51 & 0.32 & 0.62 & 0.55 \\ 
		
		UDA-SCL & 0.40 & 0.94 & 0.78 & 0.46 & 0.57 & 0.45 & 0.65 & 0.61 \\
		
		UDA-ABCL(ours) & \textbf{0.73} & 0.88 & \textbf{0.83} & 0.46 & 0.64 & 0.36 & \textbf{0.76} & 0.67 \\
		
		UDA-WeightedCE-SCL & 0.5 & \textbf{0.96} & 0.73 & \textbf{0.58} & 0.59 & \textbf{0.55} & 0.65 & 0.65 \\
		UDA-WeightedCE-ABCL(ours) & 0.68 & 0.9 & 0.79 & 0.51 & \textbf{0.67} & 0.45 & 0.74 & \textbf{0.68} \\
		
		\bottomrule
		\hline
	\end{tabular}
	\caption{ Test set recall results of the algorithms for each class of the HAM10000 dataset. The number in brackets under each class name shows the fraction of all samples belonging to that class. Therefore the major class with most examples is NV.}
	\label{tab:recall_classes}
\end{table}

~\textbf{\emph{The importance of high recall for minor classes.}} In the medical domain it is usually better to mistakenly report a false positive than to miss a true positive disease diagnosis. This is because manual assessment or further testing can be used to correct the misdiagnosis. However, missing a positive disease diagnosis may leave a potentially fatal condition untreated. Additionally, in medical data, the amount of healthy cases is usually higher than the amount of diseased cases implying the major class is usually the healthy case. In the skin cancer dataset, the NV class is the benign class, which is also the only major class and the rest are minor classes. Based on this principle, ABCL gives better performance than all its competitors. The test set results in ~\autoref{tab:recall_classes} shows that ABCL when compared to its nearest non-ABCL rival achieves higher recall for the minor classes MEL, BCC, BKL and VASC. This means ABCL is less likely to miss disease diagnosis than alternative losses.
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{ROC.png}
	\caption{Test set ROC and AUC results for each class of the HAM10000 dataset using UDA baseline, SCL and ABCL methods. The number in the brackets next to the class name is the fraction of examples that belong to that class.}
	\label{fig:ROC}
\end{figure}

\begin{table}
	\scriptsize
	\begin{tabular}{ m{1.6cm} m{0.7cm}  m{0.7cm} m{0.7cm} m{0.8cm} m{0.7cm} m{0.7cm} m{0.7cm} | m{0.9cm}  }
		\toprule
		\textbf{Algorithms} &\textbf{MEL (0.11)} &\textbf{NV (0.67)} &\textbf{BCC (0.06)} &\textbf{AKIEC (0.03)} &\textbf{BKL (0.11)} &\textbf{DF (0.01)} &\textbf{VASC (0.01)} &\textbf{Average AUC} \\
		\midrule
		UDA baseline & 0.85 & 0.91 & 0.96 & 0.91 & 0.89 & 0.89 & 0.97 & 0.91 \\
		
		UDA-ABCL(ours) & \textbf{0.93} & \textbf{0.95} & \textbf{0.98} & \textbf{0.96} &\textbf{0.95} & \textbf{0.95} & \textbf{0.99} & \textbf{0.95} \\
		
		UDA-SCL& 0.86& 0.91 & 0.97 & 0.92 & 0.89 & 0.88 & 0.98 & 0.92 \\ 
		
		\bottomrule
		\hline
	\end{tabular}
	\caption{ Test set AUC results for each class of the HAM10000 dataset and its average using UDA baseline, SCL and ABCL methods. The number in the brackets next to the class name is the fraction of examples that belong to that class.}
	\label{tab:auc}
\end{table}
~\autoref{fig:ROC} shows our ABCL method compared against the SCL and UDA baseline using the ROC and the corresponding AUC. ABCL’s AUC results are better than the UDA baseline and SCL for all classes according to ~\autoref{tab:auc}. This means ABCL is better at separating between the positive and negative classes than the alternatives.

\subsection{The effects of varying $\gamma$ value}
\para In this section we analyse the important $\gamma$ parameter of ABCL according to reported recall results for each class in ~\autoref{tab:recall_gamma}. Important observations include the following:
\begin{itemize}
	\item As $\gamma$ approaches 1, the recall of the major class NV  decreases and the recall of almost all minor classes increases.
	\item As $\gamma$ approaches 0, the recall of the major class NV  increases and the recall of almost all minor classes decreases.
\end{itemize}

This implies that as $\gamma$ is increasing, the model is compensating more towards the minor classes than the major class, leading to the degradation of major class performance. This can be explained by the case when the model correctly predicts the OSP as the major class and mispredicts the ASP as the minor class, the blended target class distribution is then skewed towards the ASP. As $\gamma$ approaches 1, the blended target class distribution moves closer to ASP. Therefore the $\gamma$ term in ABCL can be used to tradeoff decreased major class performance for increased minor class performance. 

From ~\autoref{tab:recall_gamma} we decided to choose a $\gamma$ value of 0.4 as our default value since it provided a good balance of recall for the minor classes while retaining most of the recall for the major class NV.

\begin{table}
	\scriptsize
	\begin{tabular}{m{0.8cm} m{0.8cm} m{0.8cm} m{0.8cm} m{0.8cm} m{0.8cm} m{0.8cm} m{0.8cm} | m{0.8cm}}
		\toprule
		\textbf{$\gamma$ value} &\textbf{MEL (0.11)} &\textbf{NV (0.67)} &\textbf{BCC (0.06)} &\textbf{AKIEC (0.03)} &\textbf{BKL (0.11)} &\textbf{DF (0.01)} &\textbf{VASC (0.01)} &\textbf{UAR} \\
		\midrule
		0.2 & 0.66 & \textbf{0.92} & 0.82 & 0.47 & 0.65 & 0.32 & 0.68 & 0.65 \\
		
		0.4 & 0.73 & 0.88 & 0.83 &0.46 & 0.64 & 0.36 & 0.76 & 0.67 \\ 
		
		0.5 & 0.74 & 0.86 & 0.84 & 0.51 & 0.64 & 0.41 & 0.71 & 0.67 \\ 
		
		0.6 & 0.73 &0.83 & 0.84 & 0.51 & \textbf{0.66} & 0.36 & 0.76 & 0.67 \\ 
		
		0.8 & 0.75 & 0.78 & \textbf{0.86} & 0.49 & 0.63 & \textbf{0.45} &0.76 & 0.68 \\
		
		1 & \textbf{0.78} & 0.76 & 0.83 & \textbf{0.53} & 0.64 & 0.41 & \textbf{0.82} & \textbf{0.68} \\
		\bottomrule
		\hline
	\end{tabular}
	\caption{Test set recall results for each class of the HAM10000 dataset when the $\gamma$ hyper parameter value of ABCL is varied.}
	\label{tab:recall_gamma}
\end{table}

\subsection{Ablation study}
\subsubsection{Selective versus always-on target blending}
\para Here we compare ABCL with selective target blending versus ABCL with always-on target blending using the HAM10000 dataset. In our experiments we use ABCL with always-on target blending as our default method. This means even when the original and augmented samples both are predicted as the minor or major class (cases 1 and 2 of ~\autoref{tab:4 cases}), we still blend the two samples to produce the targets. However in selective target blending we do not blend the original and augmented predictions when they both predict the minor or major class, instead in this situation we resort to the standard UDA method of just setting the target as the predicted output from the original sample.

The results in ~\autoref{tab:recall_blend_select} show that the version of ABCL that always blends targets gives higher UAR (between 0.65 and 0.68) across the entire range of $\gamma$ values. In contrast, ABCL with selective target blending performs poorly for high $\gamma$ values, especially for the major class NV. ABCL improves the model’s performance on minor classes by compensating more towards minor classes. As a consequence, in case 2 of ~\autoref{tab:4 cases} (the original and augmented samples both are predicted as the minor class), there is a harmful effect to major classes that the actual major class might be mispredicted as the minor class. Therefore, in this case, always selecting the original distribution as the target distribution might exacerbate this harmful effect. On the other hand, ABCL with always-on blending can mitigate this harmful effect, leading to less degradation in the recall for the major class.


\begin{table}
	\scriptsize
	\begin{tabular}{ m{1.4cm} m{0.7cm} m{0.7cm} m{0.7cm} m{0.7cm} m{0.8cm} m{0.7cm} m{0.7cm} m{0.7cm}  | m{0.7cm}}
		\toprule
		\textbf{Algorithms} & \textbf{$\gamma$ value} &\textbf{MEL (0.11)} &\textbf{NV (0.67)} &\textbf{BCC (0.06)} &\textbf{AKIEC (0.03)} &\textbf{BKL (0.11)} &\textbf{DF (0.01)} &\textbf{VASC (0.01)} &\textbf{UAR} \\
		\midrule
		
		\multicolumn{1}{c  }{\multirow{6}{0.7cm}{ ABCL (always-on blending)} }  & 0.2 & 0.66 & \textbf{0.92} & 0.82 & 0.47 & 0.65 & 0.32 & 0.68 & 0.65 \\
		
		\multicolumn{1}{ c  }{}  & 0.4 & 0.73 & 0.88 & 0.83 &0.46 & 0.64 & 0.36 & 0.76 & 0.67 \\ 
		
		\multicolumn{1}{ c }{}  & 0.5 & 0.74 & 0.86 & 0.84 & 0.51 & 0.64 & 0.41 & 0.71 & 0.67 \\ 
		
		\multicolumn{1}{ c }{}  & 0.6 & 0.73 &0.83 & 0.84 & 0.51 & \textbf{0.66} & 0.36 & 0.76 & 0.67 \\ 
		
		\multicolumn{1}{ c }{}  & 0.8 & 0.75 & 0.78 & \textbf{0.86} & 0.49 & 0.63 & 0.45 &0.76 & 0.68 \\
		
		\multicolumn{1}{ c }{} & 1 & \textbf{0.78} & 0.76 & 0.83 & 0.53 & 0.64 & 0.41 & \textbf{0.82} & \textbf{0.68} \\
		
		\midrule
		
		\multicolumn{1}{c  }{\multirow{6}{0.7cm}{ ABCL (selective blending)} }  & 0.2 & 0.52 & 0.91 & 0.77 & 0.49 & 0.60 & 0.45 & 0.65 & 0.63 \\
		
		\multicolumn{1}{ c  }{}  & 0.4 & 0.65 & 0.83 & 0.83 &0.49 & 0.62 & \textbf{0.55} & 0.74 & 0.67 \\ 
		
		\multicolumn{1}{ c }{}  & 0.5 & 0.64 & 0.80 & 0.85 & 0.50 & 0.61 & 0.53 & 0.72 & 0.66 \\ 
		
		\multicolumn{1}{ c }{}  & 0.6 & 0.65 &0.69 & 0.85 & 0.46 & 0.55 & 0.45 & 0.76 & 0.63 \\ 
		
		\multicolumn{1}{ c }{}  & 0.8 & 0.69 & 0.53 & \textbf{0.86} & 0.53 & 0.58 & 0.32 &0.76 & 0.61 \\
		
		\multicolumn{1}{ c }{} & 1 & 0.59 & 0.50 & 0.82 & \textbf{0.56} & 0.59 & 0.41 & 0.71 & 0.60 \\
		
		\bottomrule
	\end{tabular}
	\caption{ Test set recall results selective target blending versus always-on blending for each class of the HAM10000 dataset. }
	\label{tab:recall_blend_select}
\end{table}

\subsubsection{Weak versus strong data augmentation}
\label{sec:weak_strong}
\begin{table}
	\begin{tabular}{c c c c}
		\toprule
		\textbf{Algorithms} & \textbf{UAR} & \textbf{G-mean} & \textbf{Average AUC}\\ 
		\midrule
		UDA baseline + WeakAug & 0.59 & 0.56 & 0.91 \\
		UDA baseline + StrongAug & 0.61 & 0.56 & 0.92 \\
		ABCL + WeakAug & \textbf{0.67} & \textbf{0.62} & \textbf{0.95} \\
		ABCL + StrongAug & 0.50 & 0.42 & 0.91 \\
		\bottomrule
		
	\end{tabular}
	\caption{ Test set UAR, G-mean and average AUC results of the HAM10000 dataset comparing UDA baseline and ABCL with strong data augmentation and weak data augmentation.}
	\label{tab:strongweak}
\end{table}
\para In this section we compare the effects of different data augmentation strategies for the baseline UDA method and our ABCL method on the HAM10000 dataset.~\autoref{tab:strongweak} shows the results of this experiment. The results show that for the UAR, G-mean and average AUC metrics, strong data augmentation works better than weak data augmentation for the UDA baseline whereas the opposite is true for ABCL. As discussed in ~\autoref{sec:data_augmentation}, we believe the reason for this is when using strong data augmentation, even samples belonging to major classes may be predicted wrongly since the augmentation can make very significant changes to the appearance of the images. Consequently, the main assumption behind ABCL is violated when strong data augmentation is used. The results also show that ABCL with weak data augmentation is able to outperform the baseline UDA using the strong data augmentation. This is an important result since it shows ABCL is able to overcome any negative consequence of not being able to use strong data augmentation.

\subsection{Results for the  retinal fundus glaucoma (REFUGE) dataset}
\begin{table}
	\begin{tabular}{l c c c}
		\toprule
		\textbf{Algorithms} & \textbf{UAR} & \textbf{G-mean}   & \textbf{Average AUC}\\
		\midrule
		UDA baseline & 0.55 & 0.37 & 0.82\\
		
		UDA-WeightedCE & 0.57 & 0.43 & 0.83\\
		
		UDA-Focal  & 0.57 & 0.43 & 0.82\\

		UDA-SCL & 0.55 & 0.37 & 0.81\\
		
		UDA-WeightedCE-SCL & 0.55 & 0.37 & 0.82 \\
		UDA-ABCL(ours) & 0.55& 0.37 & 0.82\\
		UDA-WeightedCE-ABCL(ours) & \textbf{0.67} & \textbf{0.61} & \textbf{0.83} \\
		\bottomrule
	\end{tabular}
	\caption{ Test set UAR, G-mean  and AUC results for the REFUGE dataset.}
	\label{tab:refuge_result}
\end{table}
\para ~\autoref{tab:refuge_result} shows the test set results of comparing ABCL with the other competing methods for the glaucoma (REFUGE) dataset. ABCL does not improve the UDA-baseline model’s performance when the standard cross entropy loss is used for the supervised loss. However, using a combination of WeightedCE for the supervised loss and ABCL for unsupervised loss, UDA-WeightedCE-ABCL is able to significantly outperform UDA-WeightedCE and UDA-WeightedCE-SCL. As explained in ~\autoref{sec:skin_resullt}, WeightedCE can help the model produce lower bias of towards the major class for the pseudo target distribution in the unsupervised consistency loss which is of benefit to both ABCL and SCL methods. However, UDA-WeightedCE-ABCL outperforms UDA-WeightedCE-SCL because ABCL is able to adaptively blend the target distribution between the original and augmented samples’s predicted distributions depending on which predicted the minor class. This helps ABCL better address the class imbalance problem in the unlabelled data.


==> Section/background.tex <==

~\section{Supervised versus Unsupervised Learning}
\para In the era of the digital world, machine learning has been playing a crucial role across many different industries and research fields such as medical research, biology, robotics, manufacturing, etc. Machine learning has been used to solve numerous problems and achieved  near human accuracy. Moreover, beyond the limitation of computation and amount of data, machine learning becomes a more powerful technique than ever. Machine learning is a subset of artificial intelligence which trains  models using data rather than explicit instructions in order to map inputs to outputs or make decisions~\cite{matthias2001learning}. Machine learning is mainly divided into three branches: supervised learning, unsupervised learning and reinforcement learning. To confine the scope of this literature survey, we will only discuss supervised and unsupervised learning. In supervised learning, a learnt model takes input data and predicts the output. The model learns the mapping from the input to the output by comparing the predicted output against the desired output. Importantly, the key requirement of supervised learning is that for every training sample, an input and desired output (known as the label) pair is provided. So, to make supervised models perform well, it is necessary to gather a large amount of labelled data. Moreover, two main categories of supervised learning are classification and regression. For classification, the output of the model should be a categorical class label. For regression, the goal is to output a numerical value. 

Another important branch of machine learning is unsupervised learning, which instead of knowing the explicit output label, it only receives the input data. The two important techniques of unsupervised learning are clustering and dimensionality reduction. The common goal of clustering is to find the pattern of a set of data points and cluster them into a group. Dimensionality reduction is the process of reducing the number of features or variables, also known as the dimension, in a dataset without impacting on the meaning of the data.
~\section{Semi-Supervised Learning}
\para The brief review of the two popular paradigms of both supervised and unsupervised learning exposes different shortcomings, for supervised learning it is expensive to obtain a large amounts of labelled data and for unsupervised learning it is hard to extract the meaningful information from unlabelled data. Thus, one promising paradigm that overcomes these obstacles is semi-supervised learning (SSL)~\cite{chapelle2009semi} which makes use of a small amount of labelled and a large amount of unlabelled data to optimize the training of models. The goal of semi-supervised learning is to learn patterns from unlabelled data and augment the prediction of the model by these patterns. More intuitively, by leveraging the unlabelled data, the model produces a better decision boundary for different classes which reflects the data’s underlying structure ~\cite{oliver2018realistic}. Over the history of machine learning, researchers have invented various approaches to semi-supervised learning which mostly refer to either transductive learning or inductive learning. Specifically, given the data set of labelled ($x_{L}$,$y_{L}$) and unlabelled $x_{U}$ data, the objective of the inductive learner is to make the prediction for any data points, whereas the transductive learner will only produce the label for unlabelled data points. In the broad perspective, the inductive semi-supervised learning generalise a model that can output the label for unseen instances, on the other hand, transductive semi-supervised learning is only able to make the label for unlabelled data, known instances, during training phase~\cite{van2020survey}. Figure~\ref{fig:SSLTaxonomy} 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLTaxonomy}
	\caption{Visualization of the semi-supervised taxonomy~\cite{van2020survey}.}
	\label{fig:SSLTaxonomy}
\end{figure}

~\section{Convolutional Neural Network For Image Classification}
\label{sec:cnn}
\para Computer vision is one of the most important domains for the application of machine learning and includes various tasks such as object detection~\cite{zhao2019object} or image classification~\cite{krizhevsky2012imagenet}, etc. Recently, many researchers have achieved state of the art results for these tasks on public datasets such as ImageNet~\cite{deng2009imagenet}, CIFAR 10 or  CIFAR 100~\cite{krizhevsky2009learning}. To achieve such successful results, almost all of them have used one breakthrough type of neural networks, called Convolutional Neural Networks (CNNs)~\cite{lecun1990handwritten,lecun1998gradient}. This type of model has the ability to help the machine understand the representation of image better and also automatically learn features from the image.
\begin{figure}
	\centering
	\includegraphics[width=.8\textwidth]{CNN}
	\caption{Inside Convolutional Neural Networks ~\cite{lecun2015deep}.}
	\label{fig:CNN}
\end{figure}

Specifically, the architecture of CNNs is designed as a series of blocks and followed by a classification module~\cite{lecun2010convolutional}. Each block contains three layers: filter bank layer, non-linearity layer and pooling layer. In addition, the main characteristic of CNNs is the feature map which is the input and output of layers in each block. For example in Figure~\ref{fig:CNN}, the very first layer receives the RGB image of a dog and outputs features of the image such as eyes, ears, etc. The filter bank layer is a set of filters, which are matrices of weights having dimensions (width,height) or (width,height,depth) corresponding to input of black and white image or color image respectively. Each filter scans through the image and makes the sum of element-wise operation with each scanned portion of the image. Intuitively, the filter is a window, which slides horizontally from top left to bottom right of the image and returns the feature map output, as shown in Figure~\ref{fig:FilterOperation}. In addition, the filter often is called a feature detector and its weights sometimes is predefined to reflect what features it wants to detect such as vertical or horizontal edge.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{FilterOperation}
	\caption{The example of filter over the image~\cite{yamashita2018convolutional}.}
	\label{fig:FilterOperation}
\end{figure}

Moreover, two important settings of filter banks are padding and stride. Padding is the process of adding zero pixels around the border of an image. Sometimes, the filter does not fit well with the image, that means the filter would be missing some parts of the image. Thus, doing padding into the image makes sure the filter captures all the information from the image. Stride is the number of pixels indicating how far the filter should move from current position on the image. The output of the filter bank layer is the input of the non-linearity layer which consists of an activation function. Most researchers use the Rectified Non-Linear Unit (ReLU)~\cite{nair2010rectified} which returns the direct input if it is not negative, otherwise returns zero. The purpose of non-linear activation function is to prevent the model from becoming a linear model and help the model to deal with the complex task. The last layer of CNNs block is the pooling layer which also uses the approach of scanning images. It applies the specific function with the filter size (width,height) as the parameter such as max pooling, average pooling or sum pooling onto every region of feature maps. For example, applying max pooling with the filter size 2x2, the function will output the highest value of a specific region. That means, pooling layer can reduce the dimensionality of feature maps and also keep the most important information out of the region. In the higher level view, the two key benefits of CNNs are parameter sharing and sparsity of connections. With parameter sharing, a filter bank is useful in one part of the image and is probably useful in another part, thus it can reduce the parameter needed. With sparsity of connections, in each layer, each output value depends only on a small number of inputs.

Lastly, all feature maps captured from a series of blocks are flatten out into input units and fed into the classification module, called fully connected layer. This layer is like a normal neural network which outputs the score for each class. CNNs are normally back-propagated as neural networks and noticeably the weight of filters also be trained. 

~\section{Deep learning for semantic segmentation}
Image segmentation can be divided into two main tasks of semantic segmentation and instance segmentation. Semantic segmentation techniques label each pixel of an image with the class it belongs to. For example, label a pixel as belonging to a tumor or the background. Instance segmentation extends semantic segmentation by further separating  pixels based on if they belong to different instances of  the same class. Figure ~\ref{fig:Segmentation} shows an example of 2 types of segmentation.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{Segmentation}
	\caption{An example of semantic and instance segmentation~\cite{kirillov2019panoptic}.}
	\label{fig:Segmentation}
\end{figure}

From the earliest days, image segmentation techniques have centralized on traditional algorithms such as thresholding, region-growing, k-means clustering, etc. However, due to the success of deep learning models (especially CNNs), image segmentation methods have significantly improved in accuracy   via CNN based methods such as DeepLab ~\cite{chen2014semantic}, U-Net~\cite{ronneberger2015u}. To confine the scope of this review, we will focus our attention on semantic segmentation methods that use deep learning models.

As discussed in Section ~\ref{sec:cnn}, CNNs are a dominant approach in computer vision, especially in the image classification task with the ability to automatically learn features and output the class prediction for the entire image (global prediction). Therefore, researchers have adapted the deep CNN approach to solve the semantic segmentation task by making it output the class prediction for each pixel of the image (local prediction), known as the prediction mask.  Early methods  used CNNs to classify the  center pixel for a given patch of input~\cite{ciresan2012deep}. The image patch is slid across the image in order to output a prediction for each pixel of the image thus achieving the required output for semantic segmentation.  However this approach  is not efficient since the same CNN kernel is applied to the overlapping regions of nearby patches multiple times.

In order to improve the efficiency of applying CNNs to semantic segmentation, an intuitive idea ~\cite{long2015fully} is  to use fully convolutional neural networks  to process the entire image in a single pass through the CNN. To do so, the CNN architecture is modified to keep the output  size the same as the input image by using downsampling and upsampling layers within a fully convolutional neural network. This idea not only brings computational efficiency by downsampling layers but also produces the required output size using the  upsampling layers. Moreover, the approach can obtain the global spatial information of the image. Due to their  effectiveness and efficiency, fully convolutional neural networks are used in all current state of the art semantic segmentation methods. 

~\subsection{Popular existing models}
~\subsubsection{Fully convolutional networks}
Long et al ~\cite{long2015fully} proposed a fully convolutional model by modifying existing state of the art CNN classification models such as VCG16, GoogleNet. The author replaced fully connected layers with fully convolutional layers including up-sampling layers. It allows the model to process an arbitrary input image size and produce a prediction mask of the same size as the input. Figure ~\ref{fig:FCN} illustrates the model. Notably, up-sampling layers include learnable deconvolution filters that up-sampling is performed using bilinear interpolation.  Additionally, to refine semantics and spatial accuracy of the output, the author used skip of connections which combines the coarse,  high level information of feature maps in middle layers with the lower level information from the earlier layers, Figure ~\ref{fig:SkipConnection}. The methods achieved 67.2$\%$ mean IoU on PASCAL VOC 2012 ~\cite{everingham2011pascal} dataset  , establishing a new state of the art result at the time.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{FCN}
	\caption{Fully convolutional networks for semantic segmentation.~\cite{long2015fully} }
	\label{fig:FCN}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SkipConnection}
	\caption{ Skip connections : allows the model to use high level information from the middle layers to inform the final fine grained predictions.~\cite{long2015fully} }
	\label{fig:SkipConnection}
\end{figure}

~\subsubsection{ Deconvolution Network (DeConvNet)}
The Deconvolution Network (DeConvNet) is another well-known CNN based model for pixel-wise segmentation which is inspired by encoder-decoder networks. Noh et al. ~\cite{noh2015learning} have proposed a novel segmentation network consisting of the convolution network (acts like an encoder network that encodes an input image into a vector of features) and the deconvolution network (acts like an decoder network) that transforms the encoding vector of features to a dense pixel-wise class prediction map of the same size as the original image. The model architecture for DeConvNet is shown in Figure~\ref{fig:DeConvNet}. Notably, the convolution network (encoder) is not fully convolutional because it includes 2 fully connected layers which are augmented at the end to impose class-specific projection.The highlight part of this study is the deconvolution network which contains a sequence of trainable deconvolution, unpooling and rectified linear units (RELU) layers. The motivation for proposing a complete deconvolution network is the absence of real deconvotion in previous models (FCNs~\cite{long2015fully}) which is one of the main limitations. The network achieved 72.5$\%$ on PASCAL VOC 2012 dataset and outperformed all rival networks at the time.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeConvNet}
	\caption{ Overall architecture of the deconvolution network, based on the VGG 16-layer CNN model ~\cite{noh2015learning}}
	\label{fig:DeConvNet}
\end{figure}

~\subsubsection{SegNet}
Badrinarayanan et al.~\cite{badrinarayanan2017segnet} proposed an interesting fully deep convolutional Encoder-Decoder network for image segmentation, named SegNet. The network architecture is quite similar to DeconvNet which consist of the convolution network (encoder) and deconvolution network (decoder), however the author removes 2 fully connected layers of the VGG16 encoder network to make SegNet become fully convolutional. The novelty of SegNet is how the decoder network upsamples the feature maps from the encoder network. Specifically, the decoder network uses pooling indices obtained in the max-pooling step of the corresponding encoder to perform unpooling like DeconvNet, but without learnable deconvolution filters. Therefore, the upsampling stage requires no learning. After each upsampling, the upsampled maps which are sparse are convolved with trainable filters to produce dense feature maps. The network is illustrated in Figure ~\ref{fig:SegNet}.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SegNet}
	\caption{ The SegNet network architecture.~\cite{badrinarayanan2017segnet} }
	\label{fig:SegNet}
\end{figure}

~\subsubsection{UNet}
So far we have discussed popular existing models for general image segmentation. In contrast the  UNet~\cite{ronneberger2015u} was initially proposed to solve medical image segmentation and then be used in general tasks.  Ronneberger et al. ~\cite{ronneberger2015u} built a U-shaped fully convolutional network for semantic segmentation comprising a contracting path (down-sampling) to capture the context and a symmetric expanding path (up-sampling) to localize objects. The contracting path architecture is similar to a typical convolution network which obtains feature maps and reduces its resolution. While the expanding path is deconvolution network-like, that upsamples feature maps. At every upsampling layer, by using the skip connections, upsampled feature maps and the correspondingly cropped feature maps from the contracting path are concatenated. Then these concatenated feature maps are convolved by two consecutive 3 x 3 convolutional filters to halve the number of channels, hence yields U-shape network, illustrated in Figure ~\ref{fig:UNet}. 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{UNet}
	\caption{ UNet network architecture. The left is the contracting path and the right is the expanding path.~\cite{ronneberger2015u}
	}
	\label{fig:UNet}
\end{figure}

~\subsubsection{DeepLab}
\label{sec:deeplab}
Chen et al. proposed a series of DeepLab models including DeepLabv1~\cite{chen2014semantic}, DeepLabv2~\cite{chen2017deeplab}, DeepLabv3~\cite{chen2017rethinking} and DeepLabv3+~\cite{chen2018encoder}, which have become one of the most popular models for semantic segmentation.
DeepLabv1 uses a fully convolutional neural network architecture  (with VGG 16 as backbone) for semantic segmentation.  It has the two important features which are dilated convolutions in the convolutional layers and fully connected Conditional Random Field (CRF) (probabilistic graphical model) at the output stage. With no extra computational cost, dilated convolutions enlarge the receptive field of the kernel by using gaps when applying the kernel to the input.  By applying dilated convolutions, the author claims it can reduce the degree of signal downsampling, as well as condition on larger  context. Applying the fully connected CRF on the segmentation score map refines the segmentation result and achieves better object localization. As illustrated in Figure~\ref{fig:DeepLabv1}, the downsampled feature map from the fully convolutional network is first upsampled to the original image resolution using bilinear interpolation and then refined by the fully connected CRF to produce the final prediction mask. At  publication time DeepLabv1 achieved the state of the art result of 71.6$\%$ IoU at the PASCAL VOC-2012 semantic image segmentation task. 
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv1}
	\caption{ The overall model architecture of DeepLabv1.~\cite{chen2014semantic}}
	\label{fig:DeepLabv1}
\end{figure}
One year later, Chen et al.~\cite{chen2017deeplab} proposed DeepLabv2 by updating DeepLabv1 with 2 major improvements. First, DeepLabv2’s fully convolutional layers used a ResNet CNN as backbone. Second, the author also proposed atrous spatial pyramid pooling (ASPP) to robustly segment objects at multiple scales, illustrated in Figure~\ref{fig:DeepLabv2ASPP}. Specifically, the incoming convolutional feature layers are filtered using multiple parallel dilated convolutional layers with different dilated rates, hence segmenting objects as well as image context at multiple scales. This work established the new state of the art result on PASCAL VOC2012 , achieving 79.7$\%$ IoU.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv2ASPP}
	\caption{ The illustration of ASPP~\cite{chen2017deeplab}}
\label{fig:DeepLabv2ASPP}
\end{figure}
Chen et al. again updated DeepLabv2 to propose a better variant of DeepLab which is DeepLabv3~\cite{chen2017rethinking} by revisiting the use of dilated convolution and removing the use of fully connected CRF. The author experimented with DeepLabv3 with 2 main ideas:
\textbf{ Going Deeper with Atrous Convolution}, illustrated in Figure~\ref{fig:DeepLabv3Cascade} the design is to have  more blocks with atrous convolution in cascade. The dilation introduced in the convolutional kernels makes it easier to capture long range information in the deeper blocks.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3Cascade}
	\caption{  The overview of atrous convolution designed  in cascade in DeepLabv3.~\cite{chen2017rethinking}}
	\label{fig:DeepLabv3Cascade}
\end{figure}
\textbf{The modified Atrous Spatial Pyramid Pooling (ASPP)}, proposed in DeepLabv2 is illustrated in Figure~\ref{fig:DeepLabv3ASPP}. The new ASPP is added with learnable batch normalization, image-level features and 1x1 convolutions. All feature maps produced from multi-parallel dilated convolution with different rates and image-level features are concatenated and processed by the 1x1 convolution, then passed through the final 1x1 convolution to produce final logits.
DeepLabv3 achieved a significant improvement on the PASCAL VOC 2012 dataset with 85.7$\%$ IoU.		
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3ASPP}
	\caption{   The overview of new ASPP in DeepLabv3.~\cite{chen2017rethinking}}
	\label{fig:DeepLabv3ASPP}
\end{figure}

Chen et al. extended DeepLabv3 to release DeepLabv3+~\cite{chen2018encoder} by adapting the system into encoder-decoder semantic segmentation architecture and using atrous convolution layers separable. Figure~\ref{fig:DeepLabv3+} shows the architecture of DeepLabv3+.   The DeepLabv3 network is used as an encoder network with the Xception network as backbone to the fully convolutional layers and still employs the ASPP. Moreover, a new effective decoder network is added to refine the segmentation results especially for large objects. The encoding features are first upsampled using bilinear interpolation and then concatenated with the corresponding and same resolution low-level features from Xception FCNs backbone. Then these concatenated features are convolved and enlarged again to produce the final prediction map. DeepLabv3+ achieved a 3.3$\%$ improvement on the results of DeepLabv3, reaching 89$\%$ IoU on PASCAL VOC 2012 dataset.		
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{DeepLabv3+}
	\caption{   The overall encoder-decoder-like semantic segmentation network of DeepLabv3+~\cite{chen2018encoder}}
	\label{fig:DeepLabv3+}
\end{figure}

~\section{Data Augmentation For Image Classification}
\para Recently, data augmentation for images have played a very significant role in the successful training of deep CNN models which typically require a large amount of data. This is a technique of creating more images from information of existing images without changing the meaning of images, hence making the data set more diverse. Applying data augmentation helps the model frequently see more unseen data, consequently tackle the overfitting issue and make the model generalise better. Data augmentation for images is mainly divided into three groups: normal augmentation, neural network based method and augmentation search. 
~\subsection{Normal Augmentation}
\para In normal augmentation, the additional images are generated by using simple mathematical functions that transform various aspects of images such as texture, shape and color. Below we describe some of the most popular data augmentation methods:

~\textbf{Rotation} : The image is rotated clockwise or counter-clockwise by a random angle between 0 to 360 degree. This means the object in the image will be rotated but its shape will not change. Figure \ref{fig:NormalAugmentation}

~\textbf{Flipping} : We can flip the direction of the image either horizontally or vertically. That means the transformed image is horizontally or vertically symmetrical with respect to the original image. Figure \ref{fig:NormalAugmentation}

~\textbf{Shifting}: Shifting augmentation is also known as translation augmentation that moves all pixel values of the image in the left,right,top and bottom direction. In the case that the object in the image moves too far, the image may lose too much information, thus making it impossible to make a correct prediction on its label. Figure \ref{fig:NormalAugmentation}

~\textbf{Crop} : A region of the image is randomly cropped with a determined size. This technique generates new images of smaller size. Figure \ref{fig:NormalAugmentation}

~\textbf{Cutout}~\cite{devries2017improved}: Inspired by the dropout regularization technique~\cite{hinton2012improving}, cutout is the technique that randomly removes a fixed sized region from images and replaces it with random pixel values. It helps the computer vision machine model to see more simulated situations where the object in the image is partially occluded. Moreover, this technique is also relatively similar to Random Erasing~\cite{zhong2017random}. Figure \ref{fig:NormalAugmentation}

~\textbf{Colour Transformation}~\cite{shorten2019survey}: For grayscale images, each pixel contains one intensity value in the range of 0-255 inclusive. For color images, each pixel contains 3 intensity values of color channels represented in a particular color space system such as RGB (Red-Green-Blue), CMY (Cyan-Magenta-Yellow) and HSI (Hue-Saturation-Intensity). To do colour augmentation, four aspects (hue, saturation, brightness and contrast) are manipulated. The most popular methods of colour transformation are histogram equalisation, and adjusting the following: brightness, contrast, white balancing, sharpening and blurring~\cite{mikolajczyk2018data}. Figure \ref{fig:ColorAugmentation}

~\textbf{Noise Injection}~\cite{shorten2019survey}: The image is injected with an amount of noisy pixel value, usually from Gaussian noise in order to help the model to learn more robust features. Figure \ref{fig:NormalAugmentation}
\begin{figure}[h]
	\centering
	\subfloat[Original]{\includegraphics[width=0.3\textwidth]{Original}} 
	\subfloat[Rotated Image]{\includegraphics[width=0.3\textwidth]{Rotation}}
	\subfloat[Horizontal Flipped Image]{\includegraphics[width=0.3\textwidth]{Flip}}
	\qquad
	\subfloat[Top Shifted Image]{\includegraphics[width=0.3\textwidth]{Shift}}
	\subfloat[Cropped Image]{\includegraphics[width=0.2\textwidth]{Crop}}
	\subfloat[Cutout Image]{\includegraphics[width=0.3\textwidth]{Cutout}}
	\qquad
	\subfloat[Noise Injected Image]{\includegraphics[width=0.3\textwidth]{Noise}}
	\caption{ Examples of normal augmentation method on dermatoscopic skin lesion image.} 
	\label{fig:NormalAugmentation} 
\end{figure} 
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{ColorAugmentation}
	\caption{ Examples of colour augmentation~\cite{shorten2019survey}.}
	\label{fig:ColorAugmentation}
\end{figure}
~\subsection{Neural Netwok Based Method}
\para In this method, the new image is generated from a trained neural network and it will preserve the semantic of its label.

~\textbf{Generative Adversarial Networks(GANs)}~\cite{goodfellow2014generative}: The idea of GANs is that having the generative model and the discriminative model, the discriminative model is trained with real data to be able to detect the sample data whether is real or fake. Then, the generative model is trained to pit against the trained discriminative model, that means the generative model releases the sample that is detected as real data by the discriminative model. Figure ~\ref{fig:GAN}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{GAN}
	\caption{Samples are drawn from a generator. The yellow box is the latest version of each sample~\cite{goodfellow2014generative}.}
	\label{fig:GAN}
\end{figure}
~\textbf{Neural Style Transfer}~\cite{gatys2015neural}: This technique is not only known as the creation of artistic images, but is also a very useful technique for image augmentation such that augmented images have the same content as original images but different styles. The idea is to feed two images into two CNNs, one of those contains the content for the new image and the other contains the style. The CNNs will separate and recombine the content and style in order to generate new images. Figure ~\ref{fig:NeuralTransfer}

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{NeuralTransfer}
	\caption{The artistic image B is generated by CNNs. The image A is the content image and the small image at bottom-left is style image~\cite{gatys2015neural}.}
	\label{fig:NeuralTransfer}
\end{figure}
~\subsection{Augmentation Search}
\para Manually applying many different random normal augmentation techniques to the training process at the same time makes it hard to figure out which one improves the model's performance. Thus, augmentation search algorithms automatically find an optimal data augmentation policy which determines for a given data set the best set of normal augmentation methods to use and their corresponding best settings.

~\textbf{AutoAugmentation}~\cite{cubuk2019autoaugment}: This method consists of two components: a search algorithm and a search space. The search algorithm uses a reinforcement learning algorithm which finds the best data augmentation policy from the search space. In the search space, a policy consists of many sub-policies. Moreover, each sub-policy has two normal image transformations corresponding with the probability of applying transformations and the magnitude of transformations. 

~\textbf{RandAugmentation}~\cite{cubuk2019randaugment}: AutoAugmentation is computationally expensive due to its focus on finding augmentation policies using a separate search phase performed on proxy tasks which include searching different models and dataset sizes. In contrast, RandAugmentation directly evaluates the impact of the data augmentation on the target model and dataset. This results in a much smaller search space involving the set of available operations, magnitude of all operations and just two hyperparameters (N and M) to tune. 

~\section{Imbalanced Class}
\label{sec:background_imbalance}
	
~\subsection{Image classification}
~\subsubsection{For Supervised learning}
\para Training data often do not have balanced distribution. For example fraud classification from transactional data, fraud transactions are much rarer than non fraud transactions. Another example task in healthcare is cancer detection where there are usually many more healthy samples than cancer samples. Therefore, in the testing phase,  the machine learning model mostly predicts the majority class in the training set rather than the minority class, leading to much lower accuracy for predicting the minority class.   Many methods have been proposed to address class imbalance, which can be grouped into three categories: data-level, algorithm-level and hybrid approaches~\cite{johnson2019survey}.

~\textbf{Data-level Approach}: Before feeding the data into the model during training, the dataset is resampled to create a balanced distribution across classes. This randomly reduces the number of majority class samples and  randomly increases the sampling of the minority class. However there are some downsides of these techniques, according to ~\cite{johnson2019survey} under-sampling the majority class might substantially reduce the  amount of information from the eliminated data.  Over-sampling will increase training time and may cause the model to over-fit. To overcome these downsides, several advanced sampling methods have been proposed in the literature. For under-sampling, in  ~\cite{mani2003knn,kubat1997addressing,barandela2004imbalanced}, intelligent methods are used to efficiently select which majority class samples are eliminated. For oversampling in~\cite{chawla2002smote,han2005borderline,bunkhumpornpat2009safe}, intelligent methods are used to create new artificial minority class samples from existing minority class samples.

~\textbf{Algorithm-level Approach}: Instead of resampling the data distribution, this method modifies the model’s algorithm to give more emphasis on the minority class and can be divided into 3 approaches~\cite{johnson2019survey}: new loss function, cost-sensitive learning and threshold moving. Mean False Error~\cite{wang2016training}, Focal Loss~\cite{lin2017focal}, Weighted Cross Entrpy Loss~\cite{phan2017dnn} are new loss functions that reduce the effect of majority class on the loss. In cost-sensitive learning~\cite{wang2018predicting,khan2017cost,zhang2016training}the model learns from the classification cost matrix, that means each class is assigned different costs. Lastly, in the threshold moving technique~\cite{krawczyk2015cost,chen2006decision,yu2016odoc}, the idea is to adjust the decision threshold to reduce bias on easy samples, in other words, make more correct predictions on hard samples.

~\textbf{Hybrid-level Approach}: There are several hybrid methods~\cite{he2009learning,dong2018imbalanced}that combine both of the above approaches that firstly resamples data distribution and then applies algorithmic approaches such as cost-sensitive learning.

~\subsubsection{For Semi-Supervised Learning}

\para All of the above methods which alleviate skewed data distribution only works for supervised learning where we know the labelled data distribution. It is really challenging to use a semi-supervised learning approach where the distribution of the unlabelled data is unknown.

\textbf{Suppressed Consistency Loss}: For SSL perturbation based methods,  Minsung ~\cite{hyun2020class} has proposed an algorithm level method which is Suppressed Consistency Loss (SLC). In  the imbalanced class learning environment, the decision boundary is more likely to move into the low-density areas of the minor class  with consistent regularization that causes the model to misclassify the minor class. Therefore, SLC will suppress the consistency loss of minor classes which in turn tends to push the decision boundary against the low-density areas.

~\subsection{Semantic segmentation}
\para While classification suffers from class imbalance at the whole image grain, semantic segmentation suffers from the same problem at the pixel grain. Especially in binary medical image segmentation, the number of background class pixels is often much larger foreground class pixels. The methods to deal with class imbalance in semantic segmentation are also divided into 2 main groups:  data level and algorithmic level approaches. 

\textbf{Data level}: It is difficult to use oversampling or undersampling methods developed for image classification for semantic segmentation. According to~\cite{taghanaki2019combo}, it would be meaningless to undersample an image by removing some major class pixels/voxels because it would remove a lot of information from the image.  For  patch-based segmentation approaches, there are several existing works~\cite{ciresan2012deep,milletari2017hough} that  use the patch selection algorithm to balance the number of patches from major and minor classes. 

\textbf{Algorithmic level}: Algorithmic approaches are more commonly used to address class imbalance for segmentation tasks. These methods include Weighted Cross Entropy Loss~\cite{phan2017dnn}, Focal Loss~\cite{lin2017focal}, Dice Loss~\cite{sudre2017generalised} which is built from Dice Coefficient metric and aims to maximize the similarity of two images , Tversky Loss~\cite{salehi2017tversky} which modifies Dice Coefficient metric in a way that weigh False Negative more than False Positive and pre-compute weight map for the ground truth in UNet~\cite{ronneberger2015u}.

To our knowledge there are no studies that mainly focus on dealing with class imbalance in the context of semi supervised semantic segmentation. Therefore, we address this gap in the literature.	 		


==> Section/highlights.tex <==

\begin{itemize}
	\item We identify the importance of handling class imbalance for semi-supervised classification of medical images. In contrast, no existing work explicitly addresses this problem for medical images.
	\item A new method Adaptive Blended Consistency Loss is proposed as a replacement for the consistency loss of perturbation based semi-supervised learning (SSL) algorithms in order to tackle the class imbalance problem in SSL.
	\item Our Adaptive Blended Consistency Loss outperformed the standard consistency loss and other existing methods designed for addressing the class imbalance problem in both supervised and semi-supervised learning. 
\end{itemize}

==> Section/problem_definition.tex <==

\para As a result of our thorough literature review, we found there is no prior work  addressing the class imbalance problem in semi-supervised learning of medical images for either classification or segmentation. Therefore in this thesis we will  address the class imbalance problem for both semi-supervised medical image classification and segmentation. 

Semi-supervised learning (SSL) for medical images is of practical importance. Large numbers of labelled training images are necessary for training highly accurate deep learning classification and segmentation models. However, it is costly and time-consuming for medical experts to manually annotate the required number of images at either image-level or pixel-level. Hence, semi-supervised learning is an ideal method to tackle this obstacle. It only requires a small portion of all scanned images to be labelled and automatically exploits statistical patterns from the rest.  Medical image datasets often contain studies that involve imbalanced datasets which the model trained on often favour the majority image class (usually negative cases), such as for the HAM10000 skin cancer dataset~\cite{tschandl2018ham10000} where the  majority of the images are classified as benign versus a small number of malignant images, for ChestX-ray14 dataset~\cite{wang2017chestx} where the majority of the images are for healthy lungs versus unhealthy lungs, or for the  Nerve Ultrasound segmentation dataset~\cite{nervesegmentation} where the number of background pixels is heavily larger than foreground pixels. Hence in this study we address the class imbalance issue for semi-supervised classification and segmentation of medical images. 


As stated earlier our problem of class imbalance in semi-supervised learning for medical images has not been explored directly in the past. There are still several studies of SSL medical images on skewed data distributions~\cite{yi2018unsupervised,creswell2018denoising,nie2018asdnet,zheng2019semi}  but they  are not focused on  addressing the class imbalance problem. There has also been work addressing the class imbalance problem for \textit{supervised} learning---such as resampling  ~\cite{mani2003knn,kubat1997addressing,barandela2004imbalanced,chawla2002smote,han2005borderline,bunkhumpornpat2009safe,ciresan2012deep,milletari2017hough}, loss function ~\cite{lin2017focal,phan2017dnn}, region-based loss~\cite{sudre2017generalised,salehi2017tversky}, cost-sensitive learning ~\cite{wang2018predicting,khan2017cost,zhang2016training}, threshold moving ~\cite{krawczyk2015cost,chen2006decision,yu2016odoc} and using a pre-compute weight map for ground truth~\cite{ronneberger2015u}---but none of these works study SSL. We found one study~\cite{hyun2020class} that proposed  a new loss function for addressing the class imbalance issue for SSL. However, the authors conduct their experiments on standard image datasets and as such the efficacy of their proposed approach remains unproven on medical image datasets where minimising the number of false negative predictions is extremely important. Furthermore they artificially made their datasets imbalanced by introducing synthetic skew into the class distribution. In contrast, our study will use a medical image dataset which contains a real skewed class distribution.



\para More formally we define our problem as follows. Given a set of $n$ labelled training examples $L = \{l_{1}, l_{2}, ...l_{n}\}$ and a set of $m$ unlabelled  training examples $U = \{u_{1}, u_{2}, ...u_{m} \} $, with $m >> n$. The class distribution of labels in $L$ and $U$ are highly skewed, so both class distributions have low entropy. We further assume that samples in both $L$ and $U$ are drawn from the same population, and hence the class distributions of $L$ and $U$ are similar.

For the image classification task, the aim is to train a model using both $L$ and $U$ such that the model achieves high average recall for all classes (the standard metric for judging the success of models on class imbalanced datasets). Hence we aim to maximize the unweighted average recall ( UAR) metric on a test data set of $z$ examples $T = {t_{1}, t_{2}, ...t_{z}}$. UAR is defined as follows:

\begin{equation*}
	\text{UAR} = \frac{\sum\limits_{C=1}^C Recall_{C}}{C}
\end{equation*}

For the image segmentation task, the aim is to train a model using both $L$ and $U$ such that the model achieves high dice coefficient metric for minor class ona test data set of $z$ examples $T = {t_{1}, t_{2}, ...t_{z}}$. Dice coefficient is defined as follows:

\begin{equation*}
	\text{Dice} = \frac{2 * TP}{2 * TP + FP + FN}
\end{equation*}

Further details of the UAR and Dice coefficient can be found in~\ref{sec:evaluation_metrics}.

We assume that $T$ has the same class distribution as $L$ and $U$.  By using the UAR  metric, we evaluate the model based on the contribution of all classes equally rather than favoring the major classes. Furthermore,  it will make sure the minor classes which are really important for us (normally ones with disease) get an equal share of the error metric.  Similarly the Dice Coefficient fairly measures performance of every class regardless of class distribution skew.

\para ~\textbf{\emph{Justification for assuming labelled and unlabelled data have the same class distribution}}: Our new loss function mainly depends on the information of the predicted class‘s frequency of unlabelled data. We can not measure the class distribution of the unlabelled dataset. Therefore, in our study, we assume that the class distribution of the unlabelled dataset is the same as the labelled dataset. This assumption is also supported by statistical theory. That is, the data distribution of a population can be represented by the data distribution of a uniform random sample from the population. In our problem, the labelled dataset is a sample taken from the population. We can use its class distribution to represent the population. Hence, it is reasonable to assume the unlabelled data has the same class distribution as the labelled data for a sufficiently large number of samples. 






==> Section/related.tex <==
~\section{Semi-Supervised Learning}
\label{sec:ssl}
\para Our focus is on intrinsically semi-supervised methods, a subclass of inductive semi supervised learning. In order to make use of unlabelled data, these methods often follow smoothness and low-density assumptions. The low-density assumption states that the decision boundary should pass through low-density areas in the data space. The smoothness assumption states that if two data points are close, it should have the same predicted label~\cite{chapelle2009semi}. Based on the assumption, the perturbation based method increases the robustness of the model by utilizing noise on unlabelled data. That means the original input and the input perturbed with noise should both produce the same predicted label. There are several techniques based on  this approach which recently achieved state of the art results, mostly on various classification tasks, such as Temporal Ensembling~\cite{laine2016temporal}, Mean Teacher~\cite{tarvainen2017mean}and Virtual Adversarial Training~\cite{miyato2018virtual}.

~\textbf{$\prod$-MODEL}~\cite{laine2016temporal}: Inspired by ensemble learning, the idea is to encourage the consistency of a model to two of its outputs $z$ and $\tilde{z}$, which is produced from the same input by applying different dropout and data augmentation conditions, over each batch training.  Figure~\ref{fig:Temporal} shows the learning framework. The model is learned from two losses, the supervised loss on $z$ prediction of only labelled inputs by using the cross entropy loss function and mean squared loss between the $z$ and $\tilde{z}$. On CIFAR-10 with only 4000 labels, the $\prod$-MODEL achieved an error rate of 12.36$\%$.

~\textbf{Temporal Ensembling}: This technique is built on top of the $\prod$-MODEL with the difference being the model only produces one output $z$ and the prediction $\tilde{z}$ is based on the model’s output in the previous epoch. The learning framework has shown in the same figure of $\prod$-MODEL, Figure~\ref{fig:Temporal}. After every training epoch, the model’s output $z$ is accumulated into an ensemble of outputs $Z$ by updating $Z$ ← $\alpha$$Z$ + (1$-$ $\alpha$)$z$ and calculating $\tilde{z}$ by dividing $Z$ by factor (1$-$$\alpha^t$).
By only producing one output at the time, the Temporal Ensembling learning method is faster than $\prod$-MODEL. Moreover, the output $\tilde{z}$ calculated in the previous epoch can be expected to have less noise than the one in $\prod$-MODEL. The slightly better result is reported on 4000 labels of CIFAR-10 with 12.16$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{Temporal}
	\caption{~\cite{laine2016temporal} Learning framework of $\prod$-MODEL and Temporal Ensembling method.}
	\label{fig:Temporal}
\end{figure}

~\textbf{Mean Teacher}: This technique consists of the dual student and teacher models which produce $z$ and $\tilde{z}$ prediction from all inputs X by applying two types of stochastic noise. Figure~\ref{fig:MeanTeacher} illustrates the learning framework. The weights $\theta$ of the student model is updated by the supervised loss on only labelled data of student’s output $z$  and the consistency loss which is the distance between student’s output $z$  and teacher output $\tilde{z}$ from the entire input. Whereas, the teacher’s weight $\theta$’ is updated by the exponential moving average of the student's weight over each batch training, which computed as follows: $\theta'_{t}$ = $\alpha\theta'_{t-1}$  + (1 $-$ $\alpha)\theta_{t}$. On 4000 labels of CIFAR-10 and trained on ResNet, the Mean Teacher achieved the state of the art result with 6.28$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MeanTeacher}
	\caption{~\cite{tarvainen2017mean} Learning framework of MeanTeacher method.}
	\label{fig:MeanTeacher}
\end{figure}

~\textbf{Virtual Adversarial Training}~\cite{miyato2018virtual}: Most perturbation based methods apply stochastic augmentation to the input. However, in this approach, the authors directly applied small directional noise to the corresponding input which makes the model‘s prediction change the most, also known as adversarial example ~\cite{goodfellow2014explaining}. Basically, the method is inspired by Adversarial Training~\cite{goodfellow2014explaining} which uses the following loss function: 
\begin{equation}
	L_{adv}(x_{l},\theta) := D[q(y|x_{l}),p(y|x_{l} + r_{adv},\theta)]
\end{equation}
\begin{equation}
\text{where }r_{adv}:=\operatorname*{arg\,max}_{r;||r||\leq\epsilon} D[q(y|x_{l}),p(y|x_{l} + r,\theta)]
\end{equation}
The goal of the loss function is to minimize the divergence between the true distribution of output label $q(y|x_{l})$ and the model’s output distribution $p(y|x_{l} + r_{adv},\theta)$ by applying adversarial noise $r_{adv}$ to inputs $x_{l}$. However, the adversarial training only works well on supervised tasks. To transfer to the semi-supervised task, the loss function is reformulated as:
\begin{equation}
	L(x_{*},\theta) := D[p(y|x_{*},\hat{\theta}),p(y|x_{*} + r_{adv},\theta)]
\end{equation}
\begin{equation}
\text{where }r_{adv}:=\operatorname*{arg\,max}_{r;||r||_{2}\leq\epsilon} D[p(y|x_{*},\hat{\theta}),p(y|x_{*} + r)]
\end{equation}
Where $x_{*}$ is either unlabelled $x_{u}$ or labelled $x_{l}$. Indeed, we can not obtain $q(y|x_{u})$, therefore the authors  proposed the term called virtual labels which replaces $q(y|x_{*})$ with its current output $p(y|x_{*},\hat{\theta})$. This is the reason for the use of the terms “virtual” on all of the techniques reported by the paper including virtual adversarial training, virtual adversarial noise. On 4000 labels of CIFAR-10, the Virtual Adversarial Training achieved the state of the art result with 10.55$\%$ error rate.

~\textbf{Unsupervised Data Augmentation}~\cite{xie2019unsupervised}: the authors found applying advanced data augmentation on unlabelled samples could effectively make the model more invariant to noisy input in the semi-supervised learning approach. Instead of applying only some normal data augmentations such as flip, rotation in Temporal Ensembling, Mean Teacher or virtual adversarial noise in Virtual Adversarial Training, they used an auto augmentation method called ~\textbf{RandAugmentation}~\cite{cubuk2019randaugment} to find policies and magnitudes of chosen transformations which yield the best performance on labelled samples and then apply these to unlabelled samples. As a result, on CIFAR 10 with 4000 labels, this approach achieved a 5.29$\%$ error rate which is near the state of the art result for supervised learning approach. 

~\textbf{MixMatch}~\cite{berthelot2019mixmatch}: This approach does not fully belong to perturbation based method because it just utilizes the idea of perturbation based semi-supervised method as a part of the algorithm. MixMatch unifies current dominant approaches such as perturbation based semi-supervised learning methods discussed above, entropy minimization which encourages the model to make low entropy prediction on unlabelled samples and ~\textbf{MixUp}~\cite{zhang2017mixup}, a technique that combines samples for training. Moreover, these approaches are combined to generate a new set of labelled data $X$’ and unlabelled data $U$’ with predicted labels. In more detail, firstly, apply data augmentation on a batch of labelled samples $X$ and unlabelled samples $U$, to create augmented batches $\hat{X}$ and $\hat{U}$. Then, construct the predicted labels for augmented $\hat{U}$ by applying a Sharpening function to reduce the  entropy of the average model’s predictions on augmented $\hat{U}$ Figure ~\ref{fig:MixMatch}. Next, to prepare for the MixUp step, shuffle $\hat{X}$ and $\hat{U}$ with predicted labels to create set $W$. After that, apply the MixUp function on $\hat{U}$ and a part of $W$ samples, $\hat{X}$ and the rest of $W$ samples to produce a new set of labelled data $X$’ and unlabelled data $U$’. Finally, the authors just used the standard semi-supervised learning loss framework which uses the cross entropy loss function for MixUp $X$’ model’s prediction of labelled data, L2 loss for MixUp $U$’ model’s predicted outputs on unlabelled data. With 4000 labels on CIFAR 10, this technique achieved the state of the art result of 4.95$\%$ error rate.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MixMatch}
	\caption{~\cite{berthelot2019mixmatch} Diagram of the label guessing process in MixMatch.}
	\label{fig:MixMatch}
\end{figure}

Another subcategory of intrinsically semi-supervised learning is generative models. The primary characteristic of this method is to generate new unlabelled data for classification.

~\textbf{Categorical Generative Adversarial Networks}~\cite{springenberg2015unsupervised}: The idea is to build on top of ~\textbf{GANs}~\cite{goodfellow2014generative} which consists of the discriminator and generative functions and only work on unsupervised tasks. To deal with semi-supervised tasks, the authors made an extension to the discriminator so that classifies K class for all samples from the labelled dataset and discriminates real versus fake samples from the generator. Intuitively, the job of the generator is changed from “generate samples that belong to the real dataset” to “generate samples that belong to the K class dataset”.  Additionally, cross entropy loss term is also added to penalize the error of discriminator’s prediction on real data and corresponding labels. As a result, on standard 4000 labels CIFAR, the network achieved a 19.58$\%$ error rate.

~\section{Semi supervised learning in semantic segmentation}
\para In this section, we review several popular semi-supervised semantic segmentation frameworks which combine small amounts of pixel-level labeled data with large amounts of data that are either weakly labeled or not labelled. Weak labels include bounding boxes or image-level labels.
~\subsection{Weakly- and Semi-Supervised Learning of a Deep Convolutional Network for Semantic Image Segmentation (2015)}
\para Papandreou et al.~\cite{papandreou2015weakly} propose a semi-supervised framework for semantic segmentation by using DeepLab as a segmentation network and proposing Expectation-Maximization (EM) algorithm to estimate the segmentation mask from weakly labeled data. The total loss has two components, illustrated in Figure~\ref{fig:SSLDeepLab}: one on strongly labeled data is from the prediction map produced by DeepLab network with its pixel-level annotations; another loss on weakly labeled data is from the prediction map produced by DeepLab network with its estimated pixel-level map which is generated from the EM algorithm. They conducted their experiments using the PASCAL VOC 2012 dataset, with 1400 strong labels and 9000 weak labels (image-level labels) which is generated by summarizing the pixel-level annotations. The proposed method achieved 66$\%$ IoU.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLDeepLab}
	\caption{DeepLab model training methodology using a combination of pixel-level (strong labels) and image-level (weak labels) annotations.~\cite{papandreou2015weakly}}
	\label{fig:SSLDeepLab}
\end{figure}

~\subsection{Revisiting Dilated Convolution: A Simple Approach for Weakly and Semi -Supervised Semantic Segmentation (2018)}
\para Wei et al.~\cite{wei2018revisiting} proposed the semi-supervised semantic segmentation method that uses the dilated convolutions for object localization. The training framework includes two modules using shared fully convolutional networks(FCNs) as the segmentation network backbone, shown in Figure~\ref{fig:SSLRevisiting}: 

The first module works on image-level labelled data. The proposed augmented classification network that has aVGG 16 backbone with multi-dilated convolutional (MDC) blocks  produces the dense localization map. The dense localization map is then further processed to generate the segmentation mask. This segmentation mask serves as supervision in the loss function with the segmentation mask produced by FCNs and the ground truth image-level label.

The second module is the normal supervised FCNs segmentation which employs pixel-level labeled data. The loss from two modules is combined to perform the semi-supervised learning. This method achieved 67.6 IoU on the PASCAL VOC 2012 dataset with 1400 strong labels and 9000 weak labels.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLRevisiting}
	\caption{ Diagram illustrating the semi-supervised semantic segmentation method proposed by Wei et al.~\cite{wei2018revisiting}  }
	\label{fig:SSLRevisiting}
\end{figure}

~\subsection{Adversarial Learning for Semi-Supervised Semantic Segmentation (2018)}
\label{sec:ssl_adv3}
\para Exploiting the success of GANs~\cite{goodfellow2014generative}, Hung et al.~\cite{hung2018adversarial} proposed the adversarial learning for semi-supervised semantic segmentation. The framework contains two networks, segmentation network which is DeepLabv2 and discriminator network, shown in Figure~\ref{fig:SSLAdversarial}. Instead of classifying an image as real or fake, the author designed the FCN discriminator to distinguish between the predicted probability  maps from the ground truth segmentation maps. In the semi-supervised training process, the method uses strong labeled data and unlabeled data which is a new feature in this study. When using strong labeled data, the segmentation network is trained using two loss functions: Cross-entropy loss ($L_{ce}$) on the segmentation ground truth and adversarial loss ($L_{adv}$) to fool the discriminator. When using unlabeled data, the segmentation network is trained with Cross entropy semi-supervised loss ($L_{semi}$). Specifically, the predicted segmentation map of the unlabeled image produced by the segmentation network is passed through the discriminator network to obtain the confidence map. Then, in the context of self-training, this confidence map serves as a target for the previous segmentation prediction in the $L_{semi}$ loss. Notably,  the discriminator network is only trained with the strongly labeled data. The study achieved 69.5$\%$ IoU on PASCAL VOC 2012 dataset using 1400 strong labeled images and 9000 unlabeled images.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLAdversarial}
	\caption{ Diagram illustrating the  Adversarial semi-supervised semantic segmentation framework~\cite{hung2018adversarial}  }
	\label{fig:SSLAdversarial}
\end{figure}

\subsection{Semi-Supervised Semantic Segmentation with High and Low-level Consistency (2019)}
\label{sec:ssl_adv4}
\para Mittal et al.~\cite{mittal2019semi} proposed a semi-supervised segmentation framework that contains two branches which are illustrated on Figure~\ref{fig:SSLs4GANMLMT}. Their method is called the Semi-Supervised Semantic Segmentation GAN-based network (s4GAN)  which improves the low-level details in the segmentation output using semi-supervised multi-label classification via the MeanTeacher approach.  s4GAN exploits class-level information to remove false-positive predictions from the segmentation map. The s4GAN branch consists of a DeepLabv2 segmentation network and a discriminator network. The segmentation network  acts as a generator to produce the segmentation maps from input images and is trained together with a discriminator network  responsible for distinguishing the ground truth segmentation maps from the generated ones. The segmentation network is trained with three loss functions: the Cross Entropy loss applied on the pixel level  labels; the feature matching loss and self-training loss applied on the unlabeled data. The discriminator network is trained with the original GAN loss: learns to differentiate between the real ground truth maps and the prediction segmentation maps of unlabeled data. The MLMT branch is the semi-supervised classification MeanTeacher network~\cite{tarvainen2017mean} which is backed by ResNet101 and works on both image-level labeled data and unlabeled data. Notably, the s4GAN and mean teacher network branches are trained separately. 

The output of the mean teacher network is the predicted classification score for all classes. This is then used to refine the predicted segmentation maps from s4GAN to produce the final prediction segmentation mask. The prediction segmentation mask for a particular class is removed from the maps if its classification score is less than the predefined threshold.This method achieved 71.4$\%$ IoU  on the PASCAL VOC data set using 1400 strongly labeled data samples and 9000 unlabeled data samples.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLs4GANMLMT}
	\caption{ Diagram illustrating the semi-supervised semantic segmentation method proposed by Mittal et al.~\cite{mittal2019semi} called the s4GAN + Multi-label MeanTeacher classifier.  }
	\label{fig:SSLs4GANMLMT}
\end{figure}

~\subsection{Semi-Supervised Semantic Segmentation with Cross-Consistency Training (2020)}
~\label{sec:ssl_cs5}
Ouali et al.~\cite{ouali2020semi} presented a cross-consistency based training method for semi-supervised semantic segmentation. The idea is to use the encoder-decoder as the segmentation architecture and perturbation-based approach, discussed in Section~\ref{sec:ssl}, for semi-supervised learning. Specifically, there is one encoder and one main decoder and multiple auxiliary decoders, as shown in Figure~\ref{fig:SSLMultiDecoder}. The encoder and main decoder is trained using supervised Cross Entropy loss with pixel level targets. For the unlabeled examples, the encoder and all auxiliary decoders are trained using unsupervised loss by applying a consistency loss between the main decoder predictions and all auxiliary decoder predictions which are produced from different types of noise applied to the inputs of the auxiliary decoders. Notably, the unsupervised loss is not back-propagated through the main-decoder. The study established a new state of the result of 69.4$\%$ IoU on the PASCAL VOC 2012 dataset.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{SSLMultiDecoder}
	\caption{ Semi-Supervised Encoder-Decoder Semantic Segmentation with Cross-Consistency Training~\cite{ouali2020semi}.}
	\label{fig:SSLMultiDecoder}
\end{figure}

~\subsection{Semi-supervised semantic segmentation needs strong, varied perturbations (2020)}
~\label{sec:ssl_cs6}
\para French et al.~\cite{french2020semi} proposed a perturbation based semi-supervised semantic segmentation method that uses the MeanTeacher framework~\cite{tarvainen2017mean}. The method used strong varied perturbations such as CutOut, CutMix. The segmentation network used is DeepLabv2 and DenseUnet trained on 2 losses: the supervised Cross Entropy loss on pixel-level labeled data and unsupervised consistency loss on unlabelled data. Specifically for the unlabelled data, the unsupervised consistency loss enforces the consistency between the target, which is the prediction segmentation maps of the Teacher network on the original image, and the predicted segmentation maps of the Student network. The input to the student network is strongly augmented data using methods such as CutOut and CutMix. With this simple semi-supervised framework, the study achieved 67.6$\%$ IoU on the PASCAL VOC 2012.

~\section{CNNs For Medical Image Classification}
\para Medical imaging has played a crucial diagnostic role in modern medicine. The common types of medical image can be divided as follows: Ultrasound which is the  safest method for the patient’s health and is generated by using sound waves; X-Ray which is the oldest technology and generated by using electromagnetic radiation; CT (Computer tomography) which builds the 3D image based on X-Rays; and MRI ( Magnetic Resonance Imaging) which is generated by using a strong magnetic field and radio waves~\ref{fig:MedicalImage}. Besides the four common imaging types listed above, there is another type of medical image used for skin lesions that generate dermoscopy images using skin surface microscopy. In addition, medical image is obtained to visualize the information of the internal human body in order to support pathologists, radiologists or clinicians to make a diagnosis about the disease. The final diagnosis of a patient’s health should be made by doctors based on combined evidence from various processes and scans of the patient. Manually analysing medical images for multiple patients is a laborious, repetitive task and error prone task for doctors. Therefore automated diagnosis would help doctors work more efficiently. One of the most common underlying technologies of these systems is deep learning which leverages a substantial amount of medical imaging data. Deep convolutional neural networks (CNNs) are the dominant technique for this task. There are many applications of using deep CNNs in medical imaging tasks including tumor segmentation, cancer detection, cancer classification, image guided therapy, medical image annotation, and image retrieval~\cite{anwar2018medical}. To confine the scope in this section we only describe the application and research in the area of cancer classification using supervised CNNs. The result and objective of each study can vary depending on such factors as quantity and quality of the dataset, number of classes to classify and CNN network architecture used.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{MedicalImage}
	\caption{ Medical imaging modalities~\cite{anwar2018medical}.}
	\label{fig:MedicalImage}
\end{figure}
~\subsection{Skin Cancer Classification}
\para Han et.al.~\cite{han2018classification} worked on classifying 12 skin diseases which include basal cell carcinoma, squamous cell carcinoma, intraepithelial carcinoma, actinic keratosis, seborrheic keratosis, malignant melanoma, melanocytic nevus, lentigo, pyogenic granuloma, hemangioma, dermatofibroma and wart. They used the ResNet152 CNN model~\cite{he2016deep} to train on roughly 19000 clinical images from the Asan, MED-Note and Alas dataset. They tested on the Asan test dataset which achieved 0.91, 86.4, 85.5 for AUC, Sensitivity, Specificity respectively. When using the Edinburgh test dataset, they achieved 0.89, 85.1, 81.3 for AUC, Sensitivity, Specificity respectively.

Amirreza et.al.~\cite{rezvantalab2018dermatologist} experimented on dermoscopy images (~\cite{tschandl2018ham10000}HAM10000: 10015, ~\cite{mendoncca2013ph}PH2 : 120) which includes 8 types of skin diseases: melanoma, melanocytic nevi, basal cell carcinoma, benign keratosis, actinic keratosis and intraepithelial carcinoma, dermatofibroma, vascular lesions, and atypical nevi. They tried to use 4 different CNN models pre-trained on ImageNet including:  Google’s Inception v3~\cite{szegedy2016rethinking}, InceptionResNetv2~\cite{szegedy2017inception}, ResNet152~\cite{he2016deep}, and DenseNet201~\cite{huang2017densely}. As a result, they reported that the DenseNet201 model achieved the best accuracy among the 4 models in terms of micro and macro averaged precision (89.01$\%$ - 85.24$\%$), F1 - Score (89.01$\%$ - 85.13$\%$), and ROC AUC (98.79$\%$ - 98.16$\%$), even outperforming expert dermatologists’s performance.

Bi et.al.~\cite{bi2017automatic} worked on the problem of classifying the 3 skin diseases of melanoma, seborrheic keratosis and nevus on 3600 dermoscopy images including 1600 from the ISIC Archive dataset~\cite{gutman2016skin}. The final CNN classification model is assembled from 3 separated classification models such that one outputs 3 skin disease classes and the two others output the binary classification of melanoma versus others and seborrheic keratosis versus others. The reported result on AUC is 91.5$\%$.

Achim et.al.~\cite{hekler2019superior} involved a combination of the deep learning and skin cancer experts to build a superior skin cancer classification algorithm. Firstly, a ResNet CNN model is trained on 11,444 dermoscopic images, obtained from HAM10000 and ISIC Archive, to classify 5 skin diseases. Then both the CNNs trained model and dermatologists of German university hospitals will classify 300 test biopsy-verified images. Finally, a gradient boosting method is used to produce a new classifier from the confident outputs of the CNN model and the dermatologists. This method achieved accuracy, sensitivity and specificity results of  (82.95$\%$, 89$\%$, 84$\%$), compared to standalone dermatologists test results of  (42.94$\%$, 66$\%$, 62$\%$) and CNN model results of  (81.59$\%$, 86.1$\%$, 89.2$\%$).

~\subsection{Digital Pathology Classification}
\para Digital pathology is a field that uses computer-based technology to manage information generated specimens on slides. With the evolution of Whole Slide Images (WSI) technology which transforms the specimens on glass slides into digital high resolution images, known as histopathology image, digital pathology brings a new way to potentially help pathologist’s diagnosis more efficiently by using deep learning. However, one of the challenges in applying deep learning, specifically deep CNNs on WSI, is the very high dimensionality of the input, for example millions of pixels. Therefore, besides configuration of the model, the successful deep CNNs on pathology task also heavily depend on WSI image preprocessing.

Stomach and colon cancers are common cancers that cause high numbers of deaths worldwide, and in a 2018 report, there are 782,685 and 551,269 deaths due to stomach and colon cancer respectively. In addition, new research by Osamu et.al.~\cite{iizuka2020deep} used deep learning techniques to perform histopathological classification of stomach and colon cancer. There were three classes : adenocarcinoma, adenoma and non-neoplastic. The dataset consists of 4,128 and 4,036 whole slide images (WSIs) of the stomach and colon respectively collected from Hiroshima University and Haradoi Hospital. CNN Google’s Inception v3 model is trained on millions of patches extracted from WSIs to classify the three classes above. Then a max-pooling approach and a recurrent neural network (RNN) is used to predict the final label for the particular WSI by aggregating all it’s patch predictions.The model achieved the following AUC results, 0.97 and 0.99 for gastric adenocarcinoma and adenoma, 0.96 and 0.99 for colonic adenocarcinoma and adenoma.

Lung carcinoma is also a dangerous cancer that causes death to humans and the process of histologic pattern analysis in lung carcinoma is a very significant process in lung cancer diagnoses. Jason et.al.~\cite{wei2019pathologist} collected 422 WSIs from the Dartmouth-Hitchcock Medical Center in Lebanon.They used deep CNN Resnet architecture to classify histologic patterns on resected lung adenocarcinoma WSIs. The CNN model classifies patches extracted from the given WSI into histologic subtype patterns. Then, a heuristic is used to infer predominant and minor histologic patterns for the given WSI by aggregating its patch predictions. At the testing phase combined with experts, this method achieved a kappa score of 0.525 and an agreement of 66.6$\%$ with three pathologists, slightly higher than the inter-pathologist kappa score of 0.485 and an agreement of 62.7$\%$.

Another health problem which also receives high attention from researchers is the breast cancer. Kun et.al.~\cite{fan2019deep} applied the pipeline framework, which uses the highlight from a heat-map to classify whether the WSI contains breast cancer metastases on the Camelyon-16 grand challenge dataset. Firstly, the deep CNN Google’s Inception v3 architecture is trained to classify patches extracted from WSIs as tumor or normal. Then each WSI is slided into many patches, and fed into the trained CNN to build the tumor probability heat-map. After that, a Support Vector Machine classifier is trained on WSIs’s heat-map to finally produce the label for the entire WSI. As a result,this system achieved 90.23$\%$ of AUCs.
\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{BreastCancer}
	\caption{~\cite{fan2019deep}The framework of cancer metastases detection.}
	\label{fig:BreastCancer}
\end{figure}
~\subsection{X-ray Classification}
\para X-ray image is one of the most frequently used medical imaging modality. It is used for diagnosing patients because it is cheap and quick to obtain. Therefore using deep learning to diagnose disease from X-rays is well motivated.

Worawate et.al.~\cite{ausawalaithong2018automatic} performed binary classification on the presence of lung cancer. They used a pre- trained deep CNN DenseNet architecture to firstly retrain on the ChestX-ray14 dataset (112,120 non-cancer chest X-ray images) and then fine-tuned on the JSRT dataset (247 chest X-ray images that have 100 lung cancer) in order to alleviate the problem of small samples in the target classification task. The proposed method yielded 74.43$\%$ of mean accuracy, 74.96$\%$ mean specificity and 74.68$\%$ mean sensitivity.

 Lung pneumonia is a cause of death in humans. In 2017 a group from Stanford University~\cite{rajpurkar2017chexnet}proposed CheXNets, which uses a DenseNet 121 trained on ChestX-ray14 dataset to classify X-ray images into 14 disease classes of lung pneumonia. In the testing phase, the model achieved 0.435 F1 score which outperformed the F1 score of 0.387 achieved from averaging 4 scores from radiologists.
 
 \section{Semi-Supervised Learning In Medical Imaging Classification}
 \para In the real world, doing annotations for medical imaging usually is very time consuming for the doctors, especially when the diagnosis of multiple doctors needs to be averaged. Therefore, it is practical to apply semi-supervised learning on medical imaging classification that alleviate the problem of small amounts of labelled medical images and high availability of unlabelled medical images.
 
 For skin cancer classification on ISBI and PH2 dataset, Xin et. al.~\cite{yi2018unsupervised} used ~\textbf{Categorical Generative Adversarial} networks~\cite{springenberg2015unsupervised} in a semi supervised manner to solve two tasks, the first one is to classify the real image into melanoma or benign class, the second one is to generate synthetic images that assist the training. With only 140 labelled images, the method yielded an average precision of 0.424.
 
 In another study of skin cancer classification, Antonia et.al.~\cite{creswell2018denoising} proposed a SSL approach called ~\textbf{Denoising Adversarial AutoEncoder} that combines the Adversarial Net and AutoEncoder Net. Unlabelled samples are utilized in the generative and decoder part to help the model learn the representation of skin cancer such as color, shape and texture. labelled samples are encoded by the encoder and then are classified as either benign or malignant by the discriminator. Due to the heavy class imbalance (0.9,0.1), the classification loss is weighted for each class. On the ISIC dataset with 5000 labelled samples, the SSL approach achieved 0.82 for sensitivity and 0.85 for specificity.
 
 In the study of nucleus classification task, Hai et. al.~\cite{su2019local} integrated the current state of the art SSL approach of MeanTeacher~\cite{tarvainen2017mean} and the graph, which is generated by the Label Propagation algorithm~\cite{zhou2004learning}, that transfers the label information from labelled samples to unlabelled samples. Then the student model is learnt from classification loss, consistency loss and Siames loss which is based on the graph. On the MoNuseg dataset of 22462 nuclei including 4 types of nucleus Epithelial, Inflammatory, Fibroblast and Miscellaneous, the model yielded 75.79 for F1 score using only 10$\%$ of the labelled samples from the dataset.
 
 Moreover, Wenkai et. al.~\cite{yang2019dscgans} combined Semi-supervised Generative Adversarial Nets sGANs, Conditional Generative Adversarial Nets cGANs and Semi Supervised Support Vector Machine S3VM to construct the model called DScGANs (dual-path semi-supervised conditional generative adversarial networks) to solve the thyroid nodule classification task. Notably, the DScGANs is trained under conditional constraint Domain Knowledge (DK) which is acquired from the processed patches called OS, which has 225 pixel value for nodule region and 0 pixel value for non-nodule region, based on consultation with experienced radiologists. The role of DK can be summarized as follows: provide the auxiliary information to help the generator improve image quality; make the connection between information of labelled data and unlabelled data; and acts as a condition to constrain the S3VM to classify the lesion image as benign or malignant. With only 35$\%$ labelled samples from 3090 ultrasonography thyroid nodule lesion images, the proposed method achieved 90.5$\%$ for accuracy and 91.4$\%$ for AUC.
 
 \section{Semi supervised learning in medical semantic segmentation}
 \para For semantic segmentation of medical images, obtaining pixel-level annotation of 2D images or 3D volumes by medical experts is costly and time-consuming, leading  there to be much more unlabeled data compared to labelled data. Therefore, semi-supervised learning is a promising learning framework for medical images that leverages a limited amount of pixel-level labeled data and a large amount of unlabeled data.  There has been many semi supervised frameworks proposed for semantic segmentation of medical images. They can be  grouped into 2 broad types: adversarial training~\cite{nie2018asdnet,zhang2017deep,zheng2019semi,li2020shape}  and consistency training~\cite{bortsova2019semi,li2018semi,yu2019uncertainty}. These methods use the same basic methodology as those used for general semantic segmentation methods that were described  in Sections~\ref{sec:ssl_adv3},~\ref{sec:ssl_adv4} for adversarial training and Sections~\ref{sec:ssl_cs5},~\ref{sec:ssl_cs6} for consistency training.
 

